Rapid Top-Down Synthesis of Large-Scale IoT Networks

Advances in optimization and constraint satisfaction techniques, together with the availability of elastic computing resources, have spurred interest in large-scale network verification and synthesis. Motivated by this, we consider the top-down synthesis of ad-hoc IoT networks for disaster response and search and rescue operations. This synthesis problem must satisfy complex and competing constraints: sensor coverage, line-of-sight visibility, and network connectivity. The central challenge in our synthesis problem is quickly scaling to large regions while producing cost-effective solutions. We explore two qualitatively different representations of the synthesis problems satisfiability modulo convex optimization (SMC), and mixed-integer linear programming (MILP). The former is more expressive, for our problem, than the latter, but is less well-suited for solving optimization problems like ours. We show how to express our network synthesis in these frameworks, and, to scale to problem sizes beyond what these frameworks are capable of, develop a hierarchical synthesis technique that independently synthesizes networks in sub-regions of the deployment area, then combines these. We find that, while MILP outperforms SMC in some settings for smaller problem sizes, the fact that SMC's expressivity matches our problem ensures that it uniformly generates better quality solutions at larger problem sizes.

==> exp_bakup.tex <==
\section{Experiments and Analysis}
\label{sec:experiment}

In this section, we analyze the tradeoff between scale and optimality for the synthesis methods described in the previous sections.

\subsection{Methodology}
\label{s:methodology}

\parab{Alternatives we compare.} In this section, we extensively compare our SAT and SMC formulations (for brevity, in the rest of this section, we refer to these simply as SAT and SMC). In experiments, we have found that \textit{our MILP formulation scales poorly with increasingly larger problems}, even in the presence of a small number of obstacles. While it takes a few minutes to solve a $5 \times 5$ grid, it can take hours to solve a $10 \times 10$ grid with $1$ or $2$ obstacles. We have also tried a hierarchical approach using MILP, but that too does not scale well. We have left to future work to determine whether there exists a scalable MILP formulation. 

\parab{Inputs.} There are six inputs in the evaluation.
The \textit{problem space} $\mathbf{L}$ denotes the discretized grid $20 \times 20$ for which we synthesize the network. The performance of synthesis algorithms depends heavily on fraction of the problem space occupied by obstacles (\textit{obstacle extent}), and on how these obstacles are distributed across the problem space (\textit{obstacle dispersion}).
The \textit{coverage radius} $r_c$ and the \textit{communication radius} $r_s$ are inputs. Our results are sensitive to the ratio $\beta$ between the two quantities. Finally, we fix the coverage goal at $k=3$ (each grid in must be covered by at least three sensors).

\parab{Scalability and Performance.} Network synthesis methods can tradeoff performance for scalability. The scalability of network synthesis can be measured by the time taken to arrive at a good solution for a given problem size. Since we compare iterative synthesis methods, we define scalability as a constraint as follows: we allocate a fixed amount of execution time $T_e$ on a fixed computing configuration for each of our methods, and use the solution obtained by the end of that duration (or earlier if the synthesis has converged). A problem setting that does not scale will have arrived at a sub-optimal solution after $T_e$. In our experiments, we fix $T_e$ to 1 hour.

We then measure the performance of network synthesis by its \textit{coverage redundancy}. If the average number of sensors covering each location in the solution is $k_{avg}$, \textit{coverage redundancy} is $\alpha = \frac{k_{avg}}{k}$ where $k$ is the desired coverage. For example, if on average 6 sensors cover every location, but we desire 3-coverage, then coverage redundancy is 2. 

%% We have two constraint for the problem in focus.
%% \begin{enumerate}
%%     \item \textbf{Time of Execution}: We are interested in rapid synthesis of network topology. To this end, we choose a limit of an hour (arbitrary choice). If a solution takes more than an hour, we reject the solution and take the last best solution in the binary search algorithm.
%%     \item \textbf{Maximum number of available sensors}: This dictates the upper bound for the binary search with $N$.
%% \end{enumerate}

%% \parab{Performance Metric.} We define the performance evaluation metric as follows. 
%% \begin{enumerate}
%%  \item \textbf{Coverage Redundancy.} Let us denote the average number of sensor sensing each location in the network synthesis solution as $k_{avg}$.
%% The \emph{coverage redundancy} is defined as $\alpha = \frac{k_{avg}}{k}$ where $k$ is the desired coverage.
%% \end{enumerate}



    %% \item \textbf{Obstacles Percentage}: The percentage of obstacles dictates how many of the grids are occupied by obstacles. 
    %% \item \textbf{Obstacles Dispersion}: Scenarios with same percentage of obstacles can have different types of obstacles distribution from one large obstacle to many small obstacles. This will dictate the distribution of obstacle grids.

%% \textbf{Coverage Radius}: Different types of sensors will have different coverage i.e, sensing radius. For the evaluation, we choose a uniform set of sensors.   
%%  \textbf{Communication Radius}: This refers to the radio range of a device. In this set of experiments, we choose the value of communication radius to be same as the coverage radius. We have evaluated the synthesis methods for other relative ratio ($\beta$) between the coverage radius and communication radius. Due to coherent performance for different value of $\beta$, we only present results for $\beta = 1$.  
%%  \textbf{Sensing Goal, k-coverage:} We choose $k=3$ for all the experiments. This choice is guided by the concept of trilateration using three nearby sensors in the context of precise localization.

\parab{Parameters.} Two parameters control the tradeoff between scalability and coverage redundancy. The \textit{Grid Granularity} controls how finely we can represent the problem space. A finer grid implies lower coverage redundancy at the expense of scalability. The \textit{Sub-area size} controls the size of sub problems in hierarchical approaches; smaller sub-areas scale better at the expense of coverage redundancy.

%% This is only applicable to the SMC approach where smaller sub-area implies lesser complexity in sub-problems. However, this might lead to sensor over-provisioning. 
%% \end{enumerate}

% \begin{figure}[!ht]
%     \centering
%     \subfloat[]{\label{fig:obspercent:1}\includegraphics[width=0.47\linewidth]{results/obs_percentage_errorstat_1.eps}}
%     \subfloat[]{\label{fig:obspercent:2}\includegraphics[width=0.47\linewidth]{results/obs_percentage_timestat_1.eps}}
%     \caption{Performance Evaluation: (1) Coverage Redundancy, and (2) Solver Runtime; for Varying Percentage of Obstacles}
%     \label{fig:obspercent}
%   \end{figure}

% \ramesh{Change obstacle percent to obstacle extent}  

\subsection{The Role of Obstacles}
\label{s:role-obstacles}

To evaluate how obstacle extent and obstacles dispersion affects the performance of the proposed SAT and SMC method, we perform a set of experiments with different combination of obstacles extents and obstacle dispersion.
To quantify the obstacle dispersion, we define $\gamma$ as the average number of adjacent grids with obstacles for each obstacle grid. $\gamma$ can theoretically vary from 0 to 8 with $\gamma = 7, 8$ being highly rare. Lower values of $\gamma$ (for a fixed obstacle extent) indicate greater obstacle dispersion. We find that for $\gamma \leq 3$, SMC almost always outperforms SAT.  
We evaluate and compare the performance of SAT and SMC  for all combination of four different obstacle extents:  5\%, 15\% 25\%, 50\%; and seven different values of $\gamma = \{0,1,2,3,4,5,6\}$.
In each case, obstacles are uniformly distributed across a $20\times20$ grid. 
We set coverage radii to 6 units and explore sensitivity of results to three differnt choices of, $\beta = \{2, 1, 0.5\}$.

\parab{Obstacle Extent.}
To evaluate how obstacle extent affects the performance of the proposed SAT and SMC method, we perform a set of experiments with five different obstacle extents: 2.5\%, 5\%, 15\% 25\%, 50\%. 

%% We randomly choose the obstacles grids in a $20\times20$ space with grid size of 1 unit.\footnote{We use `unit' instead of meters or feet as the findings are equivalent for any metric used as long as everything use the same unit.}

\figref{fig:obspercent:1} illustrates that for scenarios with few obstacles (roughly $\leq 15\%$), SMC outperforms SAT method by more than a factor of 2. On the other hand, for highly obstructed environments, SAT has slightly higher coverage redundancy but runs much faster than SMC. In most cases, coverage redundancy of both solutions is around 2. \ramesh{What is the explanation for this? With $k=3$, we should have a reasonable chance to have a connected network, so this redundancy does not arise simply from having more sensors to ensure connectivity, right?} \pradipta{We discussed this in the meeting. Reminder to write something about the explanantion.}

Two reasons explain the variation in SAT performance. First, SAT's visibility and communication graphs are denser is less obstructed environments (\secref{sec:proposed-sat}), so it takes longer to find good solutions. Under restricted solution times (as in our evaluations), SAT's solutions are sub-optimal. Second, in more obstructed environments, SMC takes longer because it has to reason over more constraints. In contrast, SAT converges faster to  solutions with lower coverage redundancy in these settings both because its visibility approximation is less in obstructed environments, and because the visibility graphs are less dense.

%% The reasons behind the bad performance of SAT in low percentage of obstacles can be attributed to two factors: (1) With more number open (non-obstacle) grids, the search space for the solution increases and to return a solution in time SAT opts for a less optimal solution. This is evident from the time statistics presented in \figref{fig:obspercent:2}. (2) With larger percentage of obstacles, the visibility approximation converges more with the reality as illustrated in \figref{fig:obspercentillus:1}. On the other hand, for small percentage of obstacles the visibility approximation over-restricts the solution space (illustrated in \figref{fig:obspercentillus:2}). 


\begin{figure}[!ht]
    \centering
    \subfloat[]{\label{fig:obspercentillus:1}\includegraphics[width=0.35\linewidth]{images/ob_percent_ill_1.eps}}\qquad
    \subfloat[]{\label{fig:obspercentillus:2}\includegraphics[width=0.35\linewidth]{images/ob_percent_ill_2.eps}}
    \caption{Illustration of Over-approximation in Highly Clustered and Less Cluttered Settings. The shaded region illustrated the non-visible region in the SAT model.}
    \label{fig:obspercentillus}
\end{figure}

% \ramesh{The dispersion experiment isn't perfect, since we go from 4 obstacles to 100 obstacles. If time permits, have a better spaced size of obstacles? Also, the factor $\gamma$ is introduced suddenly and doesn't appear in the figures. We should make $\gamma$ be the x-axis in \figref{fig:obs_dist}(a)?}
 

\begin{figure}[!ht]
    \centering
    \subfloat[$\beta = 2$]{ \label{fig:heat1}\includegraphics[width=\linewidth]{results/heatmap_2.png}}\,
    \subfloat[$\beta = 1$]{\label{fig:heat2}\includegraphics[width=\linewidth]{results/heatmap_1.png}} \,
    \subfloat[$\beta = 0.5$]{\label{fig:heat3}\includegraphics[width=\linewidth]{results/heatmap_3.png}}
    \caption{Performance Comparison Heatmap For Different Combinations of obstacles extend, $\beta$ and $\gamma$. \textcolor{blue}{Blue} $\implies$ SMC performs significantly better, \textcolor{green}{Green} $\implies$ SAT performs significantly better, \textcolor{orange}{Orange} $\implies$ SAT and SMC perform within 10\% of each other, and \textcolor{yellow}{Yellow} $\implies$ absence of test scenario.}
\end{figure}

\parab{Obstacle Dispersion.}
In this experiment, we fixed the obstacle extent at 25\%, but varied the size and distribution of obstacles, ranging from obstacles the size of a single grid element to a single large obstacle covering 100 grid elements, 2 obstacles of 50 grid elements each, and 4 obstacles of 25 grid elements each.
%% To verify whether the performance statistics regarding obstacle percentage is valid for different distributions of obstacles, we performed another set of experiment with 4 different obstacle distribution in a $20 \times 20$ grid space with grid granularity of $1\times1$.
%% In the four scenarios, we place multiple obstacles of uniform size spanning multiple consecutive grids: $10\times10$, $7\times 7$, $5\times 5$, and $1\times 1$, respectively, with a total obstacle percentage of  $25\%$ in all four cases.
For this set of experiments, we choose a communication and coverage radius of 6 units, or  $\beta = 1$. 

\figref{fig:obs_dist} shows that SAT has lower coverage redundancy under lower obstacle dispersion, but, when obstacles are more dispersed, then SMC's coverage redundancy is significantly better than that of SAT. Across the entire range of dispersion SMC's coverage redundancy is within a factor of 2 of the optimal. With many small sized obstacles, SAT under-approximates visibility significantly (\figref{fig:obspercentillus:2}) and ends up placing more sensors. Thus, even with a large obstacle extent, if obstacles are small and widely dispersed, SAT's performance degrades.

%% This result suggest that even with high percentage of obstacles,  if the obstacles are very sparsely placed i.e., the average size of the obstacles are small, then SAT performs much worse compared to SMC.

%% regardless of the distribution of obstacles, the SMC methods performs consistently with nearly 2-approximations in terms of coverage redundancy. The SAT method performs slightly better for larger blocks of obstacles and perform really bad for obstacles of size $1\times 1$. This actually attributes to the visibility approximation with obstacles (\secref{sec:proposed-sat}). With many small size obstacles, the SAT method under-approximates the visibility by a large factor (illustrated in \figref{fig:obspercentillus:2}) and ends up placing more sensors. 
%% This result suggest that even with high percentage of obstacles,  if the obstacles are very sparsely placed i.e., the average size of the obstacles are small, then SAT performs much worse compared to SMC. 

To quantify the obstacle dispersion, we define $\gamma$ as the average number of adjacent grids with obstacles for each obstacle grid. $\gamma$ can vary from 0 to 8. Lower values of $\gamma$ (for a fixed obstacle extent) indicate greater obstacle dispersion. We find that for $\gamma \leq 3$, SMC almost always outperforms SAT. 

\parab{Takeaways.}
If $\gamma \leq 3$, regardless of the obstacle extent, SMC has lower coverage redundancy. SMC should be used when the obstacle extent is $\leq 15\%$, and otherwise opt for SAT/SMC depending on the runtime preference.

\ramesh{The takeaways are a nice addition.}

\ramesh{We may not have time for this, but the ideal way to do this experiment is to evaluate the whole space (extent x dispersion) and present a table or heatmap that shows where SMC is better and where SAT is better.}

\begin{figure}[!ht]
    \centering
    \subfloat[]{ \label{fig:obs_dist}\includegraphics[width=0.5\linewidth]{results/obs_distribution_errorstat.eps}}
    \subfloat[]{\label{fig:beta}\includegraphics[width=0.5\linewidth]{results/obs_distribution_errorstat_beta.eps}}
    \caption{Performance Comparison For (a) Different Distribution of Obstacle with $\beta = 1$, and (b) For Different Value of $\beta$ with Block size of 100; with $25\%$ Obstacles}
    % for Communication Radius = Coverage Radius Ratio = 6, Grid Dimension = $1\times 1$}
\end{figure}




\subsection{Sensitivity to Experimental Settings}
\label{s:sens-exper-sett}

\parab{Varying $\beta$}. The ratio of coverage to communication radius, $\beta$, can affect the quality of the solutions. When $\beta=2$, a solution for coverage also results in a connected network. In contrast, when $\beta=0.5$, additional sensors are required for coverage to ensure connectivity. We conducted an experiment for four different values of $\beta$ : 0.5, 1, 1.5, and 2. For this set of experiments, we have explored different obstacle dispersions with a fixed 25\% obstacle extent.

\ramesh{It would be nice to understand this experiment a little more. I'm having a hard  time visualizing what happens for different values of $\beta$ especially since we have $k=3$.}

\figref{fig:beta} shows that, when we have a single large obstacle, the performance difference between SAT and SMC is consistent, with SAT producing solutions with slightly lower coverage redundancy. As discussed above, at lower values of $\beta$, higher redundancy arises from the need to ensure connectivity.

%% Note that, we only present the results for obstacle block size of 100 due to page restrictions.
%% The coverage redundancy value for $\beta = 0.5$ is larger compared to the other values of $\beta$ as the solver needs to put almost twice the number of nodes to ensure connectivity which contributes to this additional coverage redundancy. 

\parae{Takeaways.} The value of $\beta$ does not affect the relative performance between SAT and SMC.

% \begin{figure}[!ht]
%     \centering
%     \includegraphics[width=\linewidth]{results/obs_distribution_errorstat_beta_diff.eps}
%     \caption{Performance Comparison For Different Value of $\beta$ with  $25\%$ Obstacle percentage}
%     % for Communication Radius = Coverage Radius Ratio = 6, Grid Dimension = $1\times 1$}
%     \label{fig:beta}
% \end{figure}
\begin{figure}[!ht]
    \centering
    \subfloat[5\% Obstacle]{\label{fig:gridsize:1}\includegraphics[width=0.47\linewidth]{results/grid_size_errorstat_5.png}}
    \subfloat[50\% Obstacle]{\label{fig:gridsize:2}\includegraphics[width=0.47\linewidth]{results/grid_size_errorstat_50.png}}
    \caption{Performance Evaluation for Varying Grid size4. One missing bar for SAT implies it could not produce any results in time.}
    \label{fig:gridsize}
\end{figure}

\parab{Grid Granularity.}
We now explore the impact of changing grid granularity. Using the $20\times20$ problem, with two different obstacle extents $5\%$ and $50\%$,  coverage and communication radii of six units, we vary the grid granularity:
$1\times 1$, $0.67 \times 0.67$, and $0.5 \times 0.5$. This effectively changes the total number of grids from 400, to 900, and 1600.
%% We keep the deployment scenario constant ($10\times 10$ grid) with two different percentage of obstacles $5\%$ and $50\%$.
%% We again choose a coverage and communication radius of 4 unit, i.e., $\beta = 1$.

% \ramesh{In some experiments we use a $20\times20$ grid, in others a $10\times10$, and we use two different values of communication and coverage radii 6 and 4. Worth fixing if we have time. Also, should the grid results also be bar graphs?}

At lower obstacle extents (\figref{fig:gridsize}(a)), SMC's coverage redundancy increases slightly with finer grid granularities. This is because, as the grid granularity becomes smaller, SMC's subproblems have to become smaller to permit scale. This ``deeper'' hierarchy results in greater sub-optimality. SAT's coverage redundancy dramatically increases below a certain grid granularity, since the scale of the problem is too large for that approach.

When the space is half-covered with obstacles (\figref{fig:gridsize}(b)),  the performance of both approaches is more or less insensitive to the choice of grid granularities we explore. In this regime, SAT's visibility graph is less dense and it's visibility over-approximation is lower; SMC's hierarchical approach permits it to scale to finer grid granularities without loss of coverage redundancy.

%% For experiments with two different percentage of obstacles $5\%$ and $50\%$, to our surprise we observe two different trends. 

%% The results presented in \figref{fig:gridsize} shows that the performance of SMC remain almost similar with slight deterioration with finer grids. The SAT method on the other hand first improve performance and then deteriorates rapidly for $5\%$ obstacles whereas it keeps on improving for $50\%$ obstacles. While the improvement is justified, the deterioration was unpredictable in both cases. After careful analysis, we deduce that the decreasing grid size implies increasing number of grids which in turn increases the number of constraint for the SMC. To cope up with the increasing constraint, we require to increase the number of sub-problems which in turn introduces some over-provision and results in deterioration in performance.  
%% Similarly, with decreasing grid size the solution search space becomes larger and unmanageable by the SAT solvers with the time constraints and results in far-from-optimal solution. For the highly cluttered scenario with $50\%$ obstacles, decreasing grid dimension does not increase the number of grids rapidly as compared the $5\%$ case. Therefore, we can see an improving trend in case of $50\%$ obstacles. If one reduces the grid size further, the SAT approach is again likely to hit a point where it becomes non-scalable and outputs far from optimal solutions.

\parae{Takeaway.} If the number of open grids in the problem space is large (approximately $\geq 600$), the SAT method is unable to produce good solution whereas the SMC method can maintain good performance.

\ramesh{We  need to be a little careful here. The number 600 is an artifact of the computing resources that you have. Perhaps we should state this in terms of a generic threshold?}

% \parab{Hierarchy sub-problem size.}
% SMC's performance can be sensitive to the choice sub-problem size. Smaller sub-problems can enable SMC to scale better, since each sub-problem can be solved faster, and all the sub-problems can be parallelized. However, smaller subproblems can introduce additional coverage redundancy. To explore this,
% we performed another set of experiments on a $40 \times 40$ uniform grid space with grid dimension of $0.25 \times 0.25$ with randomly dispersed obstacles.
% For these experiments, we choose a coverage and communication radius of 6 unit and vary the number of sub problems from 16 to 81.

% \figref{fig:hierachy} shows that the coverage redundancy can vary from 1.5 to a little over 2, as we vary the number of sub-problems.

% %However, increasing hierachy also implies reducing complexity of each subproblem and thereby decreasing the runtime of the entire synthesis as illustrated in \figref{fig:hierachy:2}.

% \parab{Takeaway.} Smaller sub-problem implies faster synthesis but worse quality of solution.

% \ramesh{As we discussed, it might be good to omit this experiment, since it raises more questions than it answers. Unless we have a principled way to determine what the optimal size of the sub problem might be, we'd have to then explain how we chose sub problem sizes for each of our experiments.}

\begin{figure}[!ht]
    \centering
    % \subfloat[]{\label{fig:hierachy}\includegraphics[width=0.47\linewidth]{results/Errorstat_hierarchy.eps}}
    \subfloat[]{\label{fig:cover_hier}\includegraphics[width = 0.46\linewidth]{results/obs_noopt_errorstat_1.eps}}
    \caption{(a) Comparison of Performance for the Proposed SMC with and without the coverage hierarchy}
    
\end{figure}

\subsection{Impact of Optimizations}
\label{s:impact-optimizations}

\parab{SMC vs SMC without Incremental Coverage Repair.}
SMC uses incremental coverage repair to scale: rather than solve for $k=3$ coverage in each sub-problem, we first solve for $k=1$ to take advantage of the fact that neighboring subproblems will provide additional coverage. Then, we repair any missing coverage by running SMC again. To understand the  benefits of this approach, we compare it with a version of SMC that does not include coverage repair (SMC-NCR). \figref{fig:cover_hier} shows that incremental coverage repair can reduce redundancy by $2-3\times$ relative to a solution that does not incorporate this technique.
%% we can achieve upto 2-3 times better performance compared to SMC without coverage hierarchy. This performance improvement is attributed to avoiding over-provisioning in each sub-problem. 
\pradipta{Still running the experiment for 15\% obstacles.}

\parae{Takeaway.} Incremental Coverage Repair can improve the performance of original SMC upto 2-3 times  by avoiding over-provisioning.

\parab{SMC vs SMC-Conn.}
SMC also incorporates an optimization where it does not attempt to solve each subproblem both for connectivity and coverage, assuming that the coverage solution results in an almost always connected network. To understand the benefits of this approach, we compare it against an alternative (SMC-Conn) in which we do solve for both connectivity and coverage in each sub problem. Our experiment settings are similar to those previous experiments: we explore five different obstacle extents, where each obstacle is the size of a single grid element and obstacles are uniformly distributed.

For these settings, \figref{fig:smcconn:1} shows that the optimization results in better quality solutions (lower coverage redundancy). This comes at the expense of slightly higher computation times (\figref{fig:smcconn:2}): when the sub problem is not connected, it's connectivity must be repaired during the step in which all subproblems are combined together, which increases the complexity of the step.

%% This set of experiments with five different percentage of obstacles (similar to \secref{sec:percent}) shows that SMC-Conn performs slightly worse than the proposed SMC method for all the testcases (illustrated in \figref{fig:smcconn:1}). This comparably inferior performance of SMC-Conn is contributed to over-provisioning of sensors with benefit of having  larger connected components prior to recovering connectivity. On the other hand, the proposed SMC method avoid over-provisioning in each subproblem and thereby requires slightly more time in connectivity reconstruction, illustrated in \figref{fig:smcconn:2}.

\parae{Takeaway.} Ensuring connectivity in each sub-problem does not have benefit in terms of coverage redundancy but can reduce runtime.

\begin{figure}[!ht]
    \centering
    \subfloat[]{\label{fig:smcconn:1}\includegraphics[width=0.47\linewidth]{results/obs_percentage_errorstat_1_conn.eps}}
    \subfloat[]{\label{fig:smcconn:2}\includegraphics[width=0.47\linewidth]{results/obs_percentage_timestat_1_conn.eps}}
    \caption{Performance Comparison Between SMC and SMC-Conn for Varying Percentage of Obstacles}
    \label{fig:smcconn}
\end{figure}

\subsection{Real World Problem Spaces}
\label{s:real-world-settings}

To understand the relative performance of  different approaches for network synthesis, we have presented results from synthetic problem spaces. In this section, we explore how synthesis scales to real-world problem spaces.

\parab{Baseline performance.}
We extracted discretized representations from Google Maps for three large segments of university campuses in North America: (1) 740 m $\times$ 680 m with $37\%$ of obstacles (2)  980 m $\times$ 640 m with $54\%$ of obstacles, (3) 860 m $\times$ 660 m with $35\%$ of obstacles. We use a grid size of $20~m\times20~m$ with a coverage and communication radius of 70~m following the standard ranges of Wi-Fi video surveillance cameras in outdoor settings. For each of these settings, SMC outperforms SAT in all three cases (\figref{fig:real:1}).

\parab{SAT and Hierarchy.}
These problem spaces exceed the scaling limits on SAT imposed by our hardware. To circumvent this, we introduced hierarchical synthesis to SAT as well: we apply SAT to smaller subproblems, then use the same hierarchical connectivity repair algorithm as in (\secref{s:smc-form-netw}). Hierarchical SAT is now able to scale easily to our problem spaces, but it's coverage redundancy is higher than that of SMC. This is because some of the subproblems have sparse distribution of obstacles, and SAT's under-approximation of visibility results in redundant coverage. However, Hierarchical SAT's runtime is significantly lower than SMC (\figref{fig:real:2}).

\parab{Hybrid Synthesis.}
This motivates a hybrid approach to network synthesis that tailors the synthesis method to each sub-problem. For a given sub-problem, we first analyze its obstacle extent and dispersion. When the extent is small ($\leq 15\%$), or when the obstacles are small and well-dispersed ($\gamma \leq 3$), we use SMC on the sub-problem and SAT otherwise. \figref{fig:real} shows that this approach results in coverage redundancy comparable to SMC, but has a runtime that is lower than SMC, and even comparable to SAT in one case.

%% With this observation, we developed a new hierarchical method for large maps where we combine the SMC and the SAT method. In each subproblem of the mixed hierarchical method, we first check the obstacle percentage and the obstacle sparsity ($\gamma$). If the obstacle percentage is $\leq 15\%$ (deduced in \secref{sec:percent}) or if $\gamma \leq 3$, we use SMC to solve the sub-problem and use SAT otherwise.  The results presented in \figref{fig:real} demonstrates that with the mixed approach we the coverage redundancy is similar the SMC approach whereas the runtime is smaller compared to SMC.

\parab{Takeaway.} To scale in large scale real world scenarios, we need to introduce hierarchy to the SAT methods as well. A hybrid synthesis technique that uses SMC for sub-problems with sparse obstacle extents, or small and widely dispersed obstacles, achieves low coverage redundancy with moderate runtime.

%% One can design a mixed hierarchical approach where each sub problem are solved either by SMC or SAT based on the obstacles percentage and the obstacle distribution. Such mixed approach can perform comparable to the SMC in terms of Coverage Redundancy but with almost half the synthesis time.  

\begin{figure}[!ht]
    \centering
    \subfloat[]{\label{fig:real:1}\includegraphics[width = 0.46\linewidth]{results/real_world_errorstat.eps}}
    \subfloat[]{\label{fig:real:2} \includegraphics[width = 0.46\linewidth]{results/real_world_timestat.eps}}
    \caption{ Performance Analysis in Real World Settings}
    \label{fig:real}
\end{figure}
% Comparison of Performance for the Proposed SMC and SAT method in three real world environment (1) Coverage Radius = Communication Radius = 70, Grid size = $20\ m \times 20 \ m$ (2) Coverage Radius = Communication Radius = 100, Grid size = $30\ m \times 30 \ m$

\subsection{Testbed Validation}
\label{s:small-scale-valid}

Finally, we present a small-scale validation of network synthesis. We ran the synthesizer on a small problem space, deployed a network corresponding to the output of the synthesis, and empirically determined if the connectivity and coverage requirements were satisfied. To do this, we used a testbed of 5 Raspberry Pi 3's with omnidirectional cameras mounted on top (\figref{fig:testbed}). The camera has a range (the distance at which a human can recognize a small object of standard dimensions, such as a cup) of $\approx 7\ m$. The Wi-Fi range of the device is roughly 15 meters.

We performed two experiments, one indoor, and one outdoor. In each case, we fed  a discretized representation of the problem space to the synthesizer, then placed the Raspberry Pis as directed by the synthesis output. To place the nodes accurately, we relied on relative measurements from the walls in the indoor settings and on GPS in the outdoor setting.

In the indoor experiment, the synthesized network satisfied the  coverage and connectivity requirements.

Outdoor validation was trickier for two reasons. First, the outdoor problem space was heavily occluded, and GPS errors hampered our ability to place the sensors at exactly the locations specified by the synthesizer. The SAT formulation permits flexibility in placement within an entire grid, so a SAT-synthesized network enabled us to validate coverage and connectivity. Second, the effective wireless range outdoors was smaller than that indoors, so we had to carefully profile the range and synthesize a network corresponding to this range. With this change, we were able to validate coverage and connectivity outdoors as well.

%% Conversely, the outdoor setting led us to two interesting challenges. Firstly, the well-known inaccuracies in GPS made it extremely hard to accurately place the devices near tall building. This led us to the following question: \emph{how can we make the solutions robust enough to placement errors?} Interestingly, the discretized SAT methods inherently provide robustness by using the notion of grid placement instead of point placement as in the SMC method. The SMC can also be fault tolerant if we use a lower coverage and connectivity radius than the actual values and thereby slightly overprovision the network. 
%% The second challenge was related to flaky connectivity. Using same setting as in indoor, we could not maintain connectivity in the outdoor setting. 
%% Surprisingly, in the outdoor setting the connectivity range was lower which attributed to densely deployed other wireless devices and temperature of the day. 
%% We solved the issue by taking a more conservative approach by lowering the communication radius in the problem formulation. However a proper approach would be to model the nearby Wi-Fi devices as a part of the environment which can be easily done with the help of similar SAT/SMC representation. We can also use a more complex model for connectivity such as log-normal model. However this is left as a future work.  

\begin{figure}[!ht]
    \centering
    % \subfloat[]{\label{fig:real:1} \includegraphics[width = 0.46\linewidth, height =0.5\linewidth]{results/real_world_errorstat.eps}}
     \includegraphics[width=0.47\linewidth]{images/IMG_4732.JPG}
   
    \caption{Real Testbed}
    \label{fig:testbed}
\end{figure}

\ramesh{We may want to move the summary to earlier.}
\parab{Summary.}
Three factors dictates what method to use for large scale synthesis: (1) Obstacle Percentage, (2) Obstacle Distribution ($\gamma$), and (3) Number of Open Grids ($|\mathcal{O}|$). With this, the range of choices are summarized in \tabref{tab:summary}.

\
\begin{table}[!ht]
    \centering
      \caption{Summary of the Experiments}
      \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|c|}
        \hline
        Obstacle  & Obstacle  &  \multicolumn{2}{c|}{Best Synthesis Method}  \\ \cline{3-4}
        Percentage  \% &  Distribution $\gamma$ &   $|\mathcal{O}| < 600$ &  $|\mathcal{O}| >= 600$   \\ \hline

         $ \leq 15 \%$ &   Any  & SMC  & SMC/Mixed\\ 
         Any    &   $\leq 3$ & SMC  & SMC/Mixed\\
         $ > 15 \%$    &   $> 3$ & SAT  & Hierarchical SAT/SMC/Mixed \\\hline
    \end{tabular}}
    \label{tab:summary}
\end{table}

==> milp_dimitri.tex <==

\section{A baseline MILP formulation}

Let $G_v = (V,E_v)$ and $G_c = (V,E_c)$ denote the (undirected) visibility and connectivity graphs, respectively. We introduce the decision variable $C = [C_1 , \dots, C_n]^\mathsf{T} \in \mathbb{Z}_{\geq 0}^n$, with $C_i$ corresponding to the number of sensors placed at the $i$\textsuperscript{th} node, for $i \in V$. 

The constraint for $k$ coverage can be written as
\begin{equation}
    \sum_{j \in N_i(G_v)} C_j \geq k, \quad \forall i \in V, \label{eq.MI.coverage}
\end{equation}
where $N_i(G) = \{ j \in V, (i,j) \in E \}$ denotes the neighbors of node $i \in V$ in the graph $G = (V,E)$. For notational convenience, let $G_s = (V_s,E_s) \subseteq G_c$ denote the graph corresponding to the network spanned by the deployed sensors, with $V_s = \{i \in V : C_i \geq 1\}$ and $E_s = \{(i,j) \in E_c : C_i,C_j \geq 1 \}$.

Given a graph $G = (V,E)$, let $D = \mathrm{diag}(d_1,\dots,d_n) \in \mathbb{Z}_{\geq 0}^{n \times n}$ and $A \in \mathbb{Z}_{\geq 0}^{n \times n}$ denote the degree and  adjacency matrices, respectively. We recall the fundamental result that a graph $G$ is connected if and only if the second largest eigenvalue of the Laplacian matrix $L = D - A$, hereby denoted by $\lambda_2$, is (strictly) positive. For a given graph (that is, with fixed nodes and vertices), checking whether this condition holds can be computationally challenging. In the design problem we consider in this paper further complications arise, as we are interested in imposing such a (nonconvex) connectivity constraint on graphs where the placement of nodes and edges is a design variable. Following the reduction proposed in \cite{CDC_Bayen}
the eigenvalue constraint can be expressed equivalently by the linear matrix inequality (LMI)
\begin{equation}
F(\alpha,\nu,L) := \alpha \mathbf{1} \mathbf{1}^\mathsf{T} - \nu I + L \succeq 0 \label{eq.MI.LMI}
\end{equation}
where $\alpha \in \mathbb{R}$, $\nu \in \mathbb{R}_{>0}$. The eigenvalue of interest then satisfies the bound $\lambda_2 > \nu$. In a problem where the nodes and edges of a graph are given (and constant), deciding whether the graph is connected can be accomplished by solving the LMI (\ref{eq.MI.LMI}) for the unknowns $\alpha$ and $\gamma$. This can be done in polynomial time using any convex solver applicable to semidefinite programs. If the nodes are fixed but the edges of the graph are a decision variable (as in the case considered in \cite{CDC_Bayen}), then the problem becomes combinatorial, that is, a mixed-integer semidefinite program (MISDP), as the elements $a_{ij} \in \{1,0\}$ of the adjacency matrix $A$ are also decision variables of the problem. When the placement of sensors and the structure of $G_s$ are also to be determined, it is easy to see that the connectivity of $G_s$ can be related to the positive semidefiniteness of a submatrix of $F(\alpha,\nu,L_c)$, where $L_c \in \mathbb{Z}^{n \times n}$ is the Laplacian of $G_c$. This submatrix is obtained by removing from $F(\alpha,\nu,L_c)$ the $i$\textsuperscript{th} column and row if no sensor has been placed at $i \in V$, that is, if $C_i = 0$. To express the latter logic in a form amendable to integer programming, consider the auxiliary variable $q \in \{1,0\}^n$, such that $q_i = 1$, if $C_i \geq 1$ (that is, if at least one sensor is placed at position $i \in V$), and $q_i = 0$, otherwise, for all $i \in V$. Let $M > n$ be a constant. Then, the constraints
\begin{equation}
    q_i \leq C_i, \quad C_i  \leq M  q_i, \quad \forall i \in V,     \label{eq.MI.q}
\end{equation}
describe the desired behavior for $q$. We use $q$ and the connectivity graph $G_c$ to appropriately constrain the elements $a_{ij}$ of a variable adjacency matrix $A \in \{1,0\}^{n \times n}$ corresponding to **. Let 
\begin{equation}
\begin{aligned}
  q_i + q_j &\geq 2 - 2(1-a_{ij}) \\
  q_i + q_j &\leq 1 + a_{ij}
\end{aligned}, \quad \forall (i,j) \in E_c \label{eq.MI.a1}
\end{equation}
and
\begin{equation}
    a_{ij} = 0, \quad  \forall (i,j) \notin E_c. \label{eq.MI.a2}
\end{equation}
At this point we could consider the MISDP problem of minimizing some meaningful objective, such as the number of deployed sensors $\sum_{i \in V} C_i$ or the total communication cost $\sum_{i,j \in V} a_{ij}$, subject to the constraints (\ref{eq.MI.coverage}), (\ref{eq.MI.LMI}), (\ref{eq.MI.q}), (\ref{eq.MI.a1}) and (\ref{eq.MI.a2}). However, the scalability of such an approach is expected to be significantly limited, due to the lack of specialized solvers for MISDPs and the need to resort to branch-and-bound techniques. We proceed to relax the positive semidefiniteness constraint (\ref{eq.MI.LMI}) to affine inequalities, that will ultimately yield an MILP which is more suitable to compare the newly proposed solutions against ****.  





%can only hold if at least one sensor has been placed at both the $i \in V$ and $j \in V$ nodes. By keeping the dimension and structure of $L$  the end of considering the case where the nodes are also a decision variable of the problem, one can 




%Before we proceed with the case of interest for our work with both nodes and edges being design variables, we present a relaxation to the constraint (\ref{eq.MILP.LMI}) that can streamline the solution process significantly by converting the problem to a mixed-integer linear program (MILP).

It is known that a matrix $M = M^T \in \mathbb{R}^{n \times n}$ with nonnegative diagonal elements that is also diagonally dominant, that is, it has elements $m_{ij}$, for $i,j = 1 ,\dots,n$, such that $|m_{ii}| \geq \sum_{j\neq i} |m_{ij}|$, is positive semidefinite (the opposite does not necessarily hold). This observation motivates us to consider a relaxation of the LMI (\ref{eq.MI.LMI}) to affine inequalities, the satisfaction of which implies that (\ref{eq.MI.LMI}) holds. As a result, instead of an MISDP program, the problem becomes an MILP, for which many relatively well-studied and widely used algorithms and solvers exist \cite{CPLEX,GUROBI}. %Applying the previously given 

The elements of the degree matrix are given by 
\begin{equation}
    d_i = \sum_{j \neq i} a_{ij}.
\end{equation}
Applying the previously given diagonal dominance condition to the matrix $F(\alpha,\nu,L_c)$ and proceeding with the algebra, one ultimately obtains the constraint $2d_i + 1 \geq \sum_{j \in V} q_j$, for all $i \in V$. For sufficiently large $N>0$, we can equivalently write
\begin{equation}
    0 \leq 2d_i  + 1- \sum\nolimits_{j \in V} q_j + N (1 - q_i), \quad \forall i \in V. \label{eq.MI.aff_connect}
\end{equation}

The MILP has decision variables $C$, $q$ and $A$, and its constraints are given by (\ref{eq.MI.coverage}), (\ref{eq.MI.q}), (\ref{eq.MI.a1}), (\ref{eq.MI.a2}) and (\ref{eq.MI.aff_connect}).

%With the help of the matrix $T \in \mathbb{R}^{n \times n}$ consisting of the auxiliary variables $t_{ij}$, for $i,j \in 1,\dots,n$, we have
%\begin{subequations}
%    \begin{align}
%        \alpha - \nu + d_i &\geq \sum_{i \neq j} t_{ij},\quad i \in V, \label{eq.MILP.LP1} \\
%        \alpha - a_{ij} &\leq t_{ij}, \quad (i,j) \in V \times V, i\neq j, \label{eq.MILP.LP2} \\
%        -(\alpha - a_{ij}) &\leq t_{ij} \quad (i,j) \in V \times V, i\neq j. \label{eq.MILP.LP3}
%    \end{align}
%\end{subequations}

%The final component of the MILP formulation is a technique to capture the fact that the nodes of the graph, the connectivity of which we are trying to establish, are not fixed but decision variables of the problem. 






%or (\ref{eq.MILP.LP1})-(\ref{eq.MILP.LP3})) are to be imposed on a subgraph of the original problem, determined by where sensors are actually placed. To this end, consider one more auxiliary variable $\Gamma \in \mathbb{R}^n$ subject to 
%\begin{subequations}
%    \begin{align}
 %       \alpha &\leq \gamma_i + M q_i, \\
 %       -\alpha &\leq -\gamma_i + M q_i, \\
 %       0 &\leq \gamma_i + M(1-q_i), \\
 %       \gamma_i &\leq M(1-q_i), 
 %   \end{align}
%\end{subequations}
%for all $i \in V$.
%\begin{subequations}
  %  \begin{align}
  %      M(1-q_i) \alpha - \nu + d_i &\geq \sum_{i \neq j} t_{ij}, \quad i \in V, \label{eq.MILP.LP1} \\
   %     \alpha - \gamma_j - a_{ij} &\leq t_{ij}, \quad (i,j) \in V \times V, i \neq j, \label{eq.MILP.LP2} \\
   %     -(\alpha - \gamma_j - a_{ij}) &\leq t_{ij}, \quad (i,j) \in V \times V, i \neq j, \label{eq.MILP.LP3}
 %   \end{align}
%\end{subequations}



==> milp_short.tex <==
\section{MILP formulation}
\label{s:basel-milp-form}

In this section, we briefly outline an encoding of the topology synthesis problem based on Mixed Integer Linear Programming (MILP) that is structured around the visibility and connectivity graphs described in \secref{sec:proposed-sat}. 

\parab{Coverage Constraint (C1).} By introducing an integer variable corresponding to the number of sensors placed in each grid point, we can capture the $k$-coverage requirement in a straightforward way by lower-bounding the sum of number of sensors that are visible from each distinct grid point.

\parab{Visibility (C2) and placement (C4) constraints.} We leverage the visibility graph described in \secref{sec:proposed-sat} for modeling visibility. As with the SAT approach, the MILP formulation does not require any placement constraints since it only chooses from unoccupied grids by construction.

\parab{Connectivity Constraint (C3).} 
To capture the connectivity constraint, we leverage a fundamental result that a graph $G$ is connected if and only if the second largest eigenvalue of the Laplacian matrix $L = D-A$, where $D$ is the degree matrix and $A$ is the adjacency matrix of $G$, is (strictly) positive. For a given graph (that is, with fixed nodes and vertices), checking whether this condition holds can be computationally challenging. In the topology synthesis problem further complications arise, as we are interested in imposing such a (nonconvex) connectivity constraint on graphs where the placement of nodes and edges is a design variable. Following the reduction proposed in~\cite{CDC_Bayen}, in a problem where the nodes and edges of a graph are given (and constant) the eigenvalue constraint can be expressed equivalently by a (convex) linear matrix inequality (LMI) in auxiliary scalar variables. Then, the connectivity of $G$ can be determined in polynomial time using any convex solver applicable to semidefinite programs~\cite{SDP_Vandenberghe_Boyd}. 

If the nodes are fixed but the edges of the graph are a decision variable (as in the case considered in \cite{CDC_Bayen}), then the problem becomes combinatorial, that is, a mixed-integer semidefinite program (MISDP), as the elements of the adjacency matrix $A$ are also decision variables of the problem. In our network synthesis problem, when the placement of sensors is also to be determined, the connectivity of the resulting network can be related to an LMI on a variable size matrix: its dimensions depend on the number of grid points with deployed sensors and the feasibility (or not) of edges depends on whether such edges exist in the connectivity graph.

Encoding such relationships in MILP is possible, at the expense of introducing a significant number of auxiliary integer variables. Alternatively, after some  algebra, one can obtain a MISDP, with constraints as described before and an objective that minimizes the number of sensors. But, lacking specialized MISDP solvers, we expect such a formulation to not scale well. So, we have resorted to
a further simplification: we relax the LMI constraint into affine inequalities\footnote{The LMI constraint is related to the positive semidefiniteness of a matrix. A diagonally dominant matrix, the space of which can be characterized by affine inequalities that can be part of a linear program, is positive semidefinite; the opposite does not necessarily hold.}.
This results in an MILP formulation for our problem, albeit one that may be conservative, especially on highly connected graphs.

\parab{The overall formulation.}
Putting all these together, the four key constraints can be summarized in \tabref{tab:prob_overall_milp}.

\begin{table}[!ht]
    \centering
     \caption{Summary of MILP Formulation of k-Coverage}
    %  \resizebox{0.8\linewidth}{!}{
    {\begin{tabular}{ccc}
        \hline
        Coverage  & (C1)  & Linear Program for k-Vertex Cover \\     
        Visibility & (C2)  &  Visibility Graph \\
        Connectivity & (C3)  &  LMI Relaxation for Positive Second   \\ 
        & & Smallest Eigenvalue of Graph Laplacian\\
        Placement & (C4)  & Not Required\\ \hline
    \end{tabular}}
    \label{tab:prob_overall_milp}
\end{table}

%% Despite the conservatism that this step may introduce as the connected graphs that one can describe will have relatively many links, we end up with the sought-after MILP formulation of the topology synthesis problem.

% \ramesh{Move this (commented out) para about MILP to the beginning of the results section.}
%% Based on our experiments with this MILP though, we find that the runtime of the MILP scales badly with increasingly larger problems. Indicatively, even if a problem in a $5 \times 5$ grid can be solved in few minutes, a $10 \times 10$ grid with $1$ or $2$ obstacles can take a couple of hours. Thus, we deduce that the MILP approach is not a scalable method for solving the network synthesis problem.  One can also devise a hierarchical approach to the MILP in a manner similar to the SMC approach. However, that also does not scale well based on our experimentation. A better scaling MILP method is left as a future work.

%With the help of the matrix $T \in \mathbb{R}^{n \times n}$ consisting of the auxiliary variables $t_{ij}$, for $i,j \in 1,\dots,n$, we have
%\begin{subequations}
%    \begin{align}
%        \alpha - \nu + d_i &\geq \sum_{i \neq j} t_{ij},\quad i \in V, \label{eq.MILP.LP1} \\
%        \alpha - a_{ij} &\leq t_{ij}, \quad (i,j) \in V \times V, i\neq j, \label{eq.MILP.LP2} \\
%        -(\alpha - a_{ij}) &\leq t_{ij} \quad (i,j) \in V \times V, i\neq j. \label{eq.MILP.LP3}
%    \end{align}
%\end{subequations}

%The final component of the MILP formulation is a technique to capture the fact that the nodes of the graph, the connectivity of which we are trying to establish, are not fixed but decision variables of the problem. 

%or (\ref{eq.MILP.LP1})-(\ref{eq.MILP.LP3})) are to be imposed on a subgraph of the original problem, determined by where sensors are actually placed. To this end, consider one more auxiliary variable $\Gamma \in \mathbb{R}^n$ subject to 
%\begin{subequations}
%    \begin{align}
 %       \alpha &\leq \gamma_i + M q_i, \\
 %       -\alpha &\leq -\gamma_i + M q_i, \\
 %       0 &\leq \gamma_i + M(1-q_i), \\
 %       \gamma_i &\leq M(1-q_i), 
 %   \end{align}
%\end{subequations}
%for all $i \in V$.
%\begin{subequations}
  %  \begin{align}
  %      M(1-q_i) \alpha - \nu + d_i &\geq \sum_{i \neq j} t_{ij}, \quad i \in V, \label{eq.MILP.LP1} \\
   %     \alpha - \gamma_j - a_{ij} &\leq t_{ij}, \quad (i,j) \in V \times V, i \neq j, \label{eq.MILP.LP2} \\
   %     -(\alpha - \gamma_j - a_{ij}) &\leq t_{ij}, \quad (i,j) \in V \times V, i \neq j, \label{eq.MILP.LP3}
 %   \end{align}
%\end{subequations}



==> problem.tex <==
\section{Problem Formulation and  Constraint Modeling}
\label{sec:problem}

In this section, we formulate the network synthesis problem and describe how we mathematically represent the constraints on synthesis.

\parab{Problem.}
Assume that we have a \textit{deployment region} (the area in which to deploy the network) $\mathbf{L} \subset \mathbb{R}^2$. Let $\mathbf{O}  \subset \mathbf{L}$ be the set of obstacles in the deployment region.
Suppose we have $N$ omni-directional sensors (\eg 360-degree cameras, acoustic sensors), and each sensor with location $s_{i} \in  \mathbb{R}^2$ has a sensing radius $r^s_i$ and a communication radius $r^c_{i}$.

The network synthesis problem seeks to \emph{find locations} $\mathbf{S} =\{s_{i} \in  \mathbb{R}^2  | i \in \{1,\cdots, N\}\}$ for the $N$ sensors such that:
\begin{enumerate}
\item At least $k$ sensors cover each point $l\in \mathbf{L} \setminus \mathbf{O}$.
\item The sensors form a connected network: \ie there exists a path from each node to every other node in the network.
\item The network uses as few of the $N$ sensors as possible.
\end{enumerate}

%% With these assumption, the network synthesis problems is: \emph{Given a set of $N$ sensors and the region of interest $\mathbf{L}$, what is the placement the sensors so that every location, $l\in \mathbf{L}$ is covered by at-least $k$ sensors and the network is connected, if feasible? What is the smallest values of $N$ to satisfy the requirements?}

% To simplify the rest of the description, we set $k=1$; I
% In subsequent sections, we explain the more general version of the problem.

%% Let us take $k=1$ just for illustration. To formulate the problem we need the following pieces first.

To concretely represent this synthesis problem, we need to model constraints imposed by limited sensing and communication ranges, as well as by visibility constraints in the environment. The following sub-paragraphs do this. 
\pradipta{Maybe add a sample image illustration of the objective.}

\parab{Coverage constraint (C1).}
Let $\mathrm{dist}(x_i, x_j) = \| x_i-x_j \|_2$ represent the Euclidean distance between  $x_i, x_j \in \mathbb{R}^2$, any two locations in the deployment region $\mathbf{L}$.  The predicate $\mathcal{C}(s_i, l_j): \mathbb{R}^2 \times \mathbb{R}^2 \rightarrow \{0,1\}$ represents the fact that sensor $s_i\in \mathbf{S}$ \emph{covers} location $l_j\in \mathbf{L} \setminus \mathbf{O}$: 
\begin{equation}
\label{e:coverage}
 \mathcal{C}(s_i, l_j) = \big( \mathrm{dist}(s_i,l_j) \leq r^s_i \big) \bigwedge \mathcal{B}(s_i, l_j)
\end{equation}
where $r^s_i$ is the coverage radius of the sensor $s_i$.  $ \mathcal{B}(s_i, l_j)$ is a predicate that checks whether there exist a line of sight between $s_i$ and $l_j$ (defined below). Line-of-sight visibility constraints are important for sensors such as cameras. Furthermore, in practice, cameras have finite range because of the finite resolution of the camera itself: beyond a certain distance, objects become too small to be distinguishable to the human eye~\cite{wang2004image}. 

The $k$-coverage goal then reduces to:
\begin{equation}
 \sum_{i=1}^N \mathcal{C}(s_i, l_j) \geq k  \ \ \ \forall \ \  l_j \in \mathbf{L} \setminus \mathbf{O}
\end{equation}
This ensures that at least $k$ sensors cover each location within the deployment region but not within an obstacle.

% A other two types of representation possible are convex representation and polygon representation. 
% Box representation is a subset of convex/polygon representation. 
% In general, the convex representation of obstacles would be possisimilar to the box estimation as illustrated in \figref{fig:convex}. Even convex representation might over-approximate the shape of the object which can be again compensated by sub-diving the obstacle in smaller convex objects. However, such convex representation has some challenges related the synthesis problem that we discuss later.

\parab{Environmental Visibility Constraints (C2).} Obstacles pose significant challenges for network synthesis (for brevity, henceforth we will use ``network synthesis'' to refer to the specific synthesis problem described above). We explore synthesis for planar surfaces for which it suffices to model obstacles in two dimensions. Future work can generalize this to 3-D models of the environment.

\parae{Discretizing obstacles.}
We can represent an obstacle in terms of a fine-grain polygon as illustrated in \figref{fig:poly}. However, the finer the representation of the obstacles, the less scalable the network synthesis process becomes. A single obstacle with $P$ vertices, creates $\mathcal{O}(M\cdot N \cdot P)$ constraints, where $M$ represents the set of points covered by sensors.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{images/poly_illus.png}
    %  \subfloat[]{\label{fig:convex}\includegraphics[width=0.48\linewidth]{images/convex_illus.png} 
    \caption{A complex obstacle can be modeled as a polygon, but this can be computationally difficult. We discretize space into grids and model each grid as occupied (if even a part of an obstacle overlaps with the grid) or unoccupied. Occupied grids are shaded in a dark color.}
    \label{fig:poly}
\end{figure}

To make synthesis tractable, we discretize the obstacle descriptions. Specifically, we discretize space into a uniform grid which induces
a new discretized space $\mathbf{D}$, in which each grid element $d\in\mathbf{D}$ is \textit{occupied} if an obstacle covers even a part of the element, else the element is \textit{unoccupied} (\figref{fig:poly}).

%% Such a discretization $\mathbf{D}$ is conservative since it may prevent the synthesizer from placing sensors in grid elements that are only partially occupied by obstacles. If a bounding box is infeasible or overly inaccurate, a finer grid could be created by dividing the object into adjacent objects (\figref{fig:bboxrefinedexample}). It is also possible to use a uniform size boxes for approximation of the obstacles.

%% \ramesh{Unclear which approach we use.}

%% The elements of $\mathbf{D}$ correspond to discrete grid spaces, so without loss of generality we may represent $\mathbf{D}\subseteq\mathbb{Z}^2$, with two integers $(d_1, d_2)$ describing the location of every $d\in\mathbf{D}$ in the grid space.


% \begin{equation}
% \begin{split}
%     &\mathcal{I}^d(\mathbf{x}) = \mathcal{I}^d(x,y) = \bigwedge_{c\in \{ -x^d_{min}, x^d_{max}\}} (x < c) \bigwedge_{c\in \{ -y^d_{min}, y^d_{max}\}} (y < c)
% \end{split}
% \label{eqn:halfplane}
% \end{equation}

% \ramesh{Do we use the grid coordinates $d_i$ anywhere? If not, remove it?}
% \begin{equation}
% \begin{split}
%     &\mathcal{I}^d(\mathbf{x}) = \mathcal{I}^d(x,y) \\
%     &= (x > x^d_{min}) \wedge (x < x^d_{max}) \wedge (y > y^d_{min}) \wedge (y< y^d_{max})
% \end{split}
% \label{eqn:halfplane}
% \end{equation}

Each grid element $d \in \mathbf{D}$ can be represented in 2-D space as the \textit{intersection of four half planes}: 
\begin{equation}
\begin{split}
    \mathcal{I}^d(\mathbf{x}) = \mathcal{I}^d(x,y) & = (x > x^d_{min}) \wedge (x < x^d_{max}) \\
    & \wedge (y > y^d_{min}) \wedge (y< y^d_{max})
\end{split}
\label{eqn:halfplane}
\end{equation}
The respective four physical corners are $\mathbf{L}^d = \lbrace \left(x^d_{min},  y^d_{min}\right)$, $\left(x^d_{max},  y^d_{min}\right)$, $\left(x^d_{max},  y^d_{max}\right)$, $\left(x^d_{min},  y^d_{max}\right) \rbrace$. 
Furthermore, since every $d\in\mathbf{D}$ is either occupied by an obstacle or free, $\mathbf{D}$ is the union of two disjoint sets $\mathbf{O}$ and $\mathbf{U}$, corresponding to occupied (obstacles) and unoccupied spaces, respectively.  

%% \begin{figure}[h]
%%     \centering

%%     \subfloat[]{\label{fig:bboxexample} \includegraphics[width=0.47\linewidth]{images/Obstaclewithbbox.png}}    \quad
%%     \subfloat[]{\label{fig:bboxrefinedexample}\includegraphics[width=0.47\linewidth]{images/obstaclerefinedbbox.png}}
%%     \caption{(a) Map discretization using a bounding box, which over-approximates the obstacle, but forms the basis for the grid defining the discrete space $\mathbf{D}$. (b) A more refined gridding to model a complex obstacle.}
%%     \label{fig:bboxexample}
%% \end{figure}

Discretization also simplifies the specification of coverage constraints. If a sensor $s_i$ covers the four corners of an unoccupied grid element $u_g \in \mathbf{U}$, then it covers all points within the element. 


\parae{Modeling Visibility.}
The four half-planes (\eqnref{eqn:halfplane}) of each occupied grid element can also model visibility. Let $\mathbf{L}^o_g$ represent the respective four corners of occupied grid element $o_g\in \mathbf{O}$. Then, line of sight depends upon two conditions: 
\begin{enumerate}
  \item[(v1)] This condition applies when all four vertices of an obstacle are on the same half plane created by the line joining a sensor location $s_i$ and a sensed location $l_j$ (\figref{fig:visibilityrules2:1}). If the line equation joining $s_i$, $l_j$ is $f_{ij}(\mathbf{x} =(x,y)) = 0$ then all four vertices should satisfy either $f_{ij}(\mathbf{x}) > 0$ or $f_{ij}(\mathbf{x}) < 0$, expressed as follows:
    \begin{equation}
       \mathcal{B}_1(s_i, l_j, o_g) =  \Bigg( \bigwedge_{\mathbf{x}\in \mathbf{L}^o_g} (f_{ij}(\mathbf{x}) > 0)\Bigg) \bigvee \Bigg(\bigwedge_{\mathbf{x}\in \mathbf{L}^o_g} (f_{ij}(\mathbf{x}) < 0)\Bigg)
    \end{equation}
    
    \item[(v2)] This condition applies when both the sensor location and the sensed location are on the outer half-plane of at least one obstacle face  (\figref{fig:visibilityrules2:2}). Mathematically, both points should satisfy one of the following four conditions: $x < x^o_{min}$, $x > x^o_{max}$, $y < y^o_{min}$, $y > y^o_{max}$, expressed as follows:
    
     \begin{equation}
    \begin{split}
    &\mathcal{B}_2\Big(s_i = (x_1, y_1), l_j = (x_2, y_2), o_g\Big)  = \\
    &\Big((x_1 < x^o_{min})\wedge (x_2 < x^o_{min}) \Big) \bigvee \\ 
    &\Big((x_1 > x^o_{max}) \wedge (x_2 > x^o_{max}) \Big)\bigvee   \\
    &\Big( (y_1 < y^o_{min}) \wedge (y_2 < y^o_{min})\Big) \bigvee \\
    &\Big( (y_1 > y^o_{max}) \wedge ( (y_2 > y^o_{max})\Big)
    \end{split}
    \label{eqn:visi2}
    \end{equation}
  \end{enumerate}



% \ramesh{The superscript 2 above is not really a squaring, right, so use something else?}

% \begin{equation}
%     \begin{split}
%     &\mathcal{B}_2\Big(s_i = (x_1, y_1), l_j = (x_2, y_2), o_g\Big)  = \\
%     & \bigvee_{c\in \{ x^o_{min}, - x^o_{max}\}} ((x_1 < c) \wedge (x_2 < c))\\ 
%     &\bigvee_{c\in \{ y^o_{min}, - y^o_{max}\}} ((y_1 < c) \wedge (y_2 < c))
%     \end{split}
%     \label{eqn:visi2}
%     \end{equation}


If $\mathcal{B}^o(s_i, l_j, o_g)$ is a predicate that checks whether obstacle $o_g$ does not blocks the line of sight between $s_i$ and $l_j$, then we can write:
\begin{equation}
\begin{split}
    \mathcal{B}^o(s_i, l_j, o_g) &= \mathcal{B}_1(s_i, l_j, o_g) \vee \mathcal{B}_2(s_i, l_j, o_g) \\
    \mathcal{B}(s_i, l_j) &= \bigwedge_{o_g \in \mathbf{O}} \mathcal{B}^o(s_i, l_j, o_g)
\end{split}
\label{eqn:visi}
\end{equation}
% \\
%     \mathcal{B}_{O}(s_i, l_j) &= \bigwedge_{v \in o_g} \mathcal{B}_{F}(s_i, l_j, v) \\
% \ramesh{Do we need the subscript in $B_{O}$? It would be good to see if we can simplify the notation a little bit throughout the paper}.


\begin{figure}[!ht]
    \centering
    \subfloat[]{\label{fig:visibilityrules2:1} \includegraphics[width=0.47\linewidth]{images/los_illius1.eps}} \quad
    \subfloat[]{\label{fig:visibilityrules2:2}\includegraphics[width=0.47\linewidth]{images/los_illius2.eps}}
    \caption{Two visibility conditions. Red dot signifies a sensor and Blue dot signifies a sensed location.}
    \label{fig:visibilityrules2}
\end{figure}

\parab{Network connectivity constraint (C3).} Modeling the network connectivity constraint is trickier.

Predicate $\mathcal{P}(s_i, s_j): \mathbb{R}^2 \times \mathbb{R}^2 \rightarrow \{0,1\}$ represents the direct connectivity between sensors $s_i, s_j\in \mathbf{S}$:
% \begin{equation}
%     \mathcal{P}(s_i, s_j) = \begin{cases} 1 \implies dist(s_i,s_j) \leq r^c_{i,j},   \\ 0 \implies dist(s_i,s_j) > r^c_{i,j} \mbox{\ or\ } i = j.\end{cases}
% \end{equation}
\begin{equation}
    \mathcal{P}(s_i, s_j) = \Big( dist(s_i,s_j) \leq r^c_{i,j} \Big)
\end{equation}
where $r^c_{i,j} = \min \{r^c_{i}, r^c_{j}\}$ and $r^c_{i}$ is the communication radius of sensor $s_i$. In this, we make two simplifying assumptions: that line-of-sight is not required for RF communication, and that wireless propagation follows a disk model. We have left to future work to relax these assumptions, because they can significantly impact the scaling of network synthesis. With these assumptions, and with the conservative choice of the communication radius, as we show later, we are able to synthesize functional networks that, when deployed in practice, satisfy the constraints. 

The predicate $\mathcal{P}(s_i,s_j)$ alone is not sufficient to establish \emph{network connectivity}. For this, we observe that an $N\times N$  adjacency matrix can represent the connectivity of every pair of nodes, $\mathbf{A}$ where $\mathbf{A}_{ij} = \mathcal{P}(s_i, s_j)$ $\forall i, j \in \{1, \cdots, N\}, \ \ i \neq j$ and $\mathbf{A}_{ij} = 0$ for $i=j$.
Thus, $\mathbf{A}_{ij}$ represents whether there exists a link between node $i$ and $j$. Then, $\mathbf{A}^h = \prod_{i=1}^{h} \mathbf{A} $ is the $h$-hop connectivity matrix where $\mathbf{A}^h_{ij}$ represents the number of paths of length $h$ from sensor i to sensor j. Let us now define a new matrix as follows:
\begin{equation}
    \hat{\mathbf{A}}_h = \mathbf{A} + \mathbf{A}^2 + \mathbf{A}^3 + ..... + \mathbf{A}^{h}.
    \label{eq:adjac}
\end{equation}
The $i,j$-th element of the matrix $\hat{\mathbf{A}}_h$ represents the number of paths between sensor $i$ and sensor $j$ with  $\leq h$ hops. For a network with $N$ nodes, the length of the longest path without a loop is $N-1$. So, to ensure network connectivity between every pair of two sensors $i$ and $j$, we need the following condition to hold:
\begin{equation}
    (\hat{\mathbf{A}}_{N-1})_{ij} > 0 \ \ \  \forall i,j\in \{1, \cdots, N\} \ \ \mathrm{with} \ \  i \neq j.
\end{equation}


% &\mathcal{B}_2\Big(s_i = (x_1, y_1), l_j = (x_2, y_2), o_g\Big)  = \\
%     & \bigvee_{c\in \{ x^o_{min}, - x^o_{max}\}} ((x_1 \leq c) \wedge (x_2 \leq c))\\ 
%     &\bigvee_{c\in \{ y^o_{min}, - y^o_{max}\}} ((y_1 \leq c) \wedge (y_2 \leq c))


% \begin{equation}
% \begin{split}
%     \mathcal{V}^o\big(s_i = (x,y), o_g\big) = &\bigvee_{c\in \{ x^o_{min}, - x^o_{max}\}} (x < c) \\
%         & \bigvee_{c\in \{ y^o_{min}, - y^o_{max}\}} (y < c)
% \end{split}
% % \label{eqn:visi}
% \end{equation}



\parab{Obstacles and sensor placement (C4).}
To prevent the synthesizer from placing sensors in grid elements occupied by obstacles, we can define constraints that ensure that each sensor $s_i$'s position is outside the four half planes (\eqnref{eqn:halfplane}) defined by each grid element, as follows:
\begin{equation}
\begin{split}
    \mathcal{V}^o\big(s_i = (x,y), o_g\big) &= (x < x^o_{min}) \vee (x > x^o_{max}) \vee  \\
    & (y < y^o_{min}) \vee (y > y^o_{max})
\end{split}
% \label{eqn:visi}
\end{equation}
where $x^o_{min}, x^o_{max}, y^o_{min}, y^o_{max}$ define the four halfplanes of the obstacle grid. 
If $\mathcal{V}(s_i)$ is a predicate that checks whether sensor $s_i \in \mathbf{S}$ is properly placed, then we can write:
\begin{equation}
    \mathcal{V}\big(s_i\big) = \bigwedge_{o_g \in \mathbf{O}} \mathcal{V}^o\big(s_i, o_g\big).
\label{eqn:placement}
\end{equation}

\parab{The overall formulation.}
Summarizing all the constraints, we can model the network synthesis goal of k-coverage by four main constraints as illustrated in \tabref{tab:prob_overall}.

\begin{table}[h]
    \centering
     \caption{Summary of Problem Formulation}

    \begin{tabular}{ccc}
            \hline \vspace{1ex}
        Coverage & (C1)  &  $\sum_{i=1}^N \mathcal{C}(s_i, l_j) \geq k  \ \ \ \forall \ \  l_j \in \mathbf{L} \setminus \mathbf{O} $ \\
           
        Visibility & (C2)  &  $\mathcal{B}(s_i, l_j) = \bigwedge_{o_g \in \mathbf{O}} \mathcal{B}(s_i, l_j, o_g)$\\\vspace{1ex}
            & &$\forall s_i \in \mathbf{S}$  and $l_j\in \mathbf{L} \setminus \mathbf{O}$\\ 
            
        Connectivity & (C3)  &  $(\hat{\mathbf{A}}_{N-1})_{ij} > 0 $\\ \vspace{1ex}
        & & $\ \ \  \forall i,j\in \{1, \cdots, N\} \ \ and \ \  i \neq j$\\ 
        Placement & (C4)  & $ \mathcal{V}\big(s_i\big) \ \ \  \forall s_i \in \mathbf{S}$\\ \hline
    \end{tabular}
    \label{tab:prob_overall}
\end{table}



==> proposed-sat.tex <==
\section{MILP-Based Network Synthesis}
\label{sec:proposed-sat}

In this section, we describe a scalable network synthesis method using a Mixed Integer Linear Programming (MILP) formulation. 
To use MILP for network synthesis, we need to find a \textit{MILP-encoding} of the constraints in \secref{sec:problem}.

%% To this end, we use the discretized space and for simplicity we assume that all nodes have same sensing radius $r^s$ and communication radius $r^c$.

%% The main advantage of a SAT formulation is that it permits adding boolean constraints to the formulation easily. \ramesh{It would be  good to add an example of an interesting constraint that could be expressed using boolean variables.}

%Next, we detail our SAT encoding of the k-coverage topology synthesis problem.
% It is worth mentioning that similarly to SMC (TODO: confirm that this appears after SMC section), SAT programming is dealing with constraint solving exclusively, that is, there is formally no objective function to be minimized or maximized, but only a logical combination of constraints to be satisfied. One can still use SAT in problem-specific optimization contexts (e.g. by trying to solve a problem with a variable corresponding to the objective function provided as a parameter, calling SAT as an oracle, and iterating or bisecting until the problem is not satisfiable). In the class of problems we consider in this work

\parab{Representing Coverage.}
To represent the coverage constraint C1 (\eqnref{e:coverage}) in MILP, we leverage the grid discretization and relax the definition of (a) distance and (b) visibility.

\parae{Distance relaxation.}
To reason about the constraints from \secref{sec:problem} in grid space, we first need to modify the distance function between any two grids in the unoccupied space $\mathbf{U}$ as follows:
\begin{equation}
    \mathrm{dist}'(u_i, u_j) = \max_{x_i\in \mathbf{L}^u_{i}, x_j \in  \mathbf{L}^u_{j}} \mathrm{dist}(x_i, x_j) \ \ , \  u_i, u_j \in \mathbf{U}
\end{equation}
where $\mathbf{L}^u_i$ represent the four corners of grid element $u_i\in \mathbf{U}$. This evaluates to the maximum distance between the two discrete regions. The largest distance measurements in this particular discrete space are between opposite corners of the rectangles describing $u_i$ and $u_j$. 

\parae{Visibility Relaxation (C2).}
The visibility between a sensor and a location is given by \eqnref{eqn:visi}. However, to create a MILP encoding we must remove any non-linear constraints. To this end, we assume that a sensor, located in a space directly adjacent to an obstacle, cannot sense any discrete space at or past the obstacle's position.  For example, if a sensor is in a space diagonal to an obstacle, it cannot sense any space on the vertically or horizontally opposite side of the object (\figref{fig:visibilityrules}). With this assumption we can pre-compute the visibility relation between any two grids in the system:
\begin{equation}
    \begin{split}
    \mathcal{B}'(u_i, u_j)  = \textsc{true}\  or \ \textsc{false}
    \end{split}
\end{equation}


%% The restrictions on sensor visibility due to obstacles are combined with natural sensor ranges $r_s$.  The sensed area is here under-approximated using the largest inscribed square within the circle defined by their sensing radius, and the use of a worst-case distance for coverage requires the sensing square to cover another location regardless of the sensor's placement within the discrete space $\mathbf{U}$.

\begin{figure}[h]
    \centering
    \subfloat[]{\includegraphics[width=0.40\linewidth]{images/ObstacleSide.png}} \quad
    \subfloat[]{\includegraphics[width=0.40\linewidth]{images/ObstacleDiag.png}}
    \caption{Visibility restrictions placed on the sensors in discrete space. We under-approximate visibility so the resulting assignment of discrete locations is valid for any real-valued location within the discrete region.}
    \label{fig:visibilityrules}
\end{figure}



% \pradipta{For further details on the method of computing these relations, please refer to the appendix.}

\parae{Modified Coverage Constraint (C1).} With the visibility relaxations, we can define a modified coverage function as:
\begin{equation}
\begin{split}
    \mathcal{C}'(u_i, u_j) &= \Big( \mathrm{dist}'(u_i, u_j) \leq r^s\Big) \bigwedge  \mathcal{B}'(u_i, u_j)  \\
\end{split}
\end{equation} 
where we use sensors of fixed sensing radius $r_s$ for ease of exposition (below, we describe how to generalize this to heterogeneous sensors).
To account for the discretization, instead of assuming that a sensor has visibility defined by the sensor range $r_s$, we assume its visibility is restricted to the largest inscribed square within the circle aligned to the grid axes (\figref{fig:visibilityrules}). This under-approximation ensures that we do not miss coverage, at the expense of optimality.

\parae{Transforming $k$-coverage into a graph vertex cover.}
With the modified coverage function, let us define a graph $G_v = (V, E_v)$ where vertex $i$ corresponds to a discrete region $u_i\in\mathbf{U}$.  We create an edge between vertices $i, j \in V$ when the corresponding discrete regions $u_i, u_j \in \mathbf{U}$ can ``cover'' each other, \ie $\mathcal{C}'(u_i,u_j) = \textsc{true}$.  \figref{vizgraph} illustrates this \textit{visibility graph}.  Now, \emph{the sensor $k$-coverage problem reduces to identifying if there exists a selection of vertices $S\subseteq V$ with $|S| = N$ such that every vertex (i.e., every $u\in\mathbf{U}$) is covered by at least $k$ neighboring vertices of $G_v$.} This specific formulation assumes that each grid can contain only one sensor.

\begin{figure}[h]
\centering
\includegraphics[width=0.45\linewidth]{images/Obstacle_with_connectivity_edges.png}
% \subfloat[]{\label{bipartite}\includegraphics[width=0.47\linewidth]{images/Bipartite.png}}
\caption{An example ``visibility graph", where each vertex represents a discrete region and edges exist between two vertices $u_1,u_2$ if the corresponding regions ``cover" each other, i.e. $\mathcal{C}'(u_1,u_2) = \textsc{true}$.}
\label{vizgraph}
\end{figure}


A MILP formulation of $k$-vertex cover uses only $|V| = |\mathbf{U}|$ integer variables. Consider a integer variable $n_i \in \mathbb{Z}_{\geq 0}$ associated with each $i\in V$ which represents the number of sensors to place on that grid. Now, the $k$-cover goal becomes:
\begin{equation}
    \label{sumbools1}
     \sum_{j \in N_i(G_v)}  n_j  \geq k, \quad \forall i \in V
\end{equation}
where $\mathcal{N}_i(G_v) = \{ j \in V : (i,j) \in E_v \}$ denotes the neighbors of node $i \in V$ in the graph $G_v = (V,E_v)$. This implies that for every $u_i\in\mathbf{U}$, at least $k$ sensors is places in its neighboring ($\mathcal{C}'(u_i,u_j) = \textsc{true}$) vertices. To ensure that we only place the maximum number of available sensors $N$, we need an additional constraint: $\sum_{i = 1}^{|V|} n_j \leq N$.
With this, the overall formulation in the MILP formulation becomes:

\begin{equation}
\begin{split}
\label{milp-form}
    &\min \sum_{i = 1}^{|V|} n_j \\
    &\sum_{j \in N_i(G_v)}  n_j  \geq k, \quad \forall i \in V \\
    &\sum_{i = 1}^{|V|} n_j \leq N  \ \ ,\ \ \ n_i \in \mathbb{Z}_{\geq 0} 
\end{split}
\end{equation}



\parae{Accommodating Heterogeneity.}
If the network synthesis requires each location to be covered by multiple types of sensors such as cameras and microphones, we can treat each type of sensor placement problem as a separate coverage problem and solve using~\eqnref{milp-form}. If the synthesis specifies multiple sensors of the same type (e.g., camera) but with different specifications, we can generate a separate visibility graph for each sensor specification ($t \in \{1, \cdots T\}$) as $G^t_v = (V, E^t_v)$, introduce an integer variable $n_{t, i}$ to represent the number of type $t$ sensors placed in the discrete region $u_i$, and update \eqnref{sumbools1} and \eqnref{milp-form} in a straightforward way (details omitted) to formulate the synthesis.

%% The $k$-cover and cardinality constraints then become: 

%% \begin{equation}
%%     \label{sumbools1}
%%     \begin{split}
%%         &\sum_{t = 1}^{T} \sum_{j \in \mathcal{N}_i(G^t_v)}  n_{t,j}  \geq k, \quad \forall i \in V\\
%%         & \sum_{j = 1}^{|V|} n_{t,j} \leq N^t
%%     \end{split}
%% \end{equation}


% \begin{equation}
% \label{hetero-sat}
% \begin{split}
%     &\bigwedge_{i\in V}\quad\left( \ \sum_{t = 1}^{T} \sum_{j \in \mathcal{N}_i(G^t_v)}   \ \  \sum_{z = 1}^{Z^t} b_{t, j,z} \geq k \right) \ \ and  \ \sum_{j = 1}^{|V|} \sum_{z = 1}^{Z^t} b_{t,j,z} = N^t % \ \ \ \forall t \in \{1, \cdots, T\}
% \end{split}
% \end{equation}
%Better representation of such heterogeneity is left as a future work.

\parae{Obstacles and sensor placement (C4).}
The visibility graph accommodates the placement constraints by construction.

% \parae{$k$-Coverage with fewest sensors.}
% With the above-mentioned constraints, we can invoke modern SAT solvers such as z3~\cite{z3}.  The resulting SAT output will present either a set of feasible vertices (and therefore discrete locations $u\in\mathbf{U}$) for sensor placement or state that no such configuration exists.  Now to find the minimum number of sensor ($N$) to deploy, we do a binary search, starting from a very large number (typically the number of grids times k).

%% In each step, we check if a solution is feasible. If feasible, we reduce the the value of $N$ by half and check again. If not feasible, we choose a higher value in between the last known feasible value and the current value. This is repeated until we have a value of $N$ which results in a feasible solution and all values less than $N$ are infeasible. 

\parab{Determining connectivity.}
Specifying connectivity in Boolean form is generally a computationally expensive task (\cite{jiang1995solving, de2014sat}). Therefore, SAT cannot express the connectivity constraints (C3) directly. We use a two-step  \textit{connectivity repair} algorithm to enforce connectivity after generating a topology satisfying the $k$-cover constraints. Similar to the creation of the visibility graph (see \figref{vizgraph}), we can create a \textit{connectivity graph} $G_c = (V,E_c)$, where vertex $i$ corresponds to a discrete region $u_i\in\mathbf{U}$, and edges exist between two vertices $i,j\in V$  if $\mathrm{dist}'(u_i, u_j) \leq r^c$. While we use a homogeneous communication radius of $r^c$ for simplicity, we plan to explore heterogeneity in our future work.

% Again, using this worst-case distance provides some robustness guarantees on any real placement of a sensor within the discrete region. One could also consider more complex connectivity models, where obstacles play a key role.
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.6\linewidth]{images/Collapse.png}
\end{center}
\caption{\label{collapse}An example collapse of the connectivity subgraph $G_s$ into its connected components.  In this figure, the solid red circled vertices correspond to the vertices $\mathbf{S}$ selected by the MILP algorithm.  The connected components of $G_s$ dashed black boxes, and each is mapped to a collapsed node, with edges mapped to their corresponding collapsed nodes.  In this new graph, the Steiner tree problem solution identifies the vertex in a dashed red circle as the necessary node for connectivity.}
\end{figure}

\parae{A graph-based formulation for connectivity repair.}
A selection of sensors by the SAT algorithm, $\mathbf{S}$, induces a subgraph $G_s = (V_s,E_s) \subseteq G_c$ on the connectivity graph $G_c$.  $E_s = \{(i,j) \in E_c : sum_{t = 1}^{T}  n_{t,i} \geq 1, sum_{t = 1}^{T}  n_{t,j} \geq 1 \}$ \ie each grid has at least one sensor. To satisfy the connectivity constraint, $G_s$ must be a connected graph.  Should the SAT algorithm produce a connected $G_s$, no additional work is necessary.  Otherwise, we must add additional vertices to the set $\mathbf{S}$, playing the role of relay nodes.

To determine the relay node locations, we collapse $G_s$ into its connected components.  In this process, every single disconnected node is considered ``self-connected'' and mapped to an identical node in the collapsed graph (\figref{collapse}).  Edges from $G_c$ are similarly mapped to their corresponding collapsed counterparts.  The problem of identifying a set of nodes to add to $\mathbf{S}$ to make $G_s$ connected is identical to finding the minimal weight tree in the collapsed graph which spans the collapsed nodes of $G_s$.

This is the Steiner tree problem in graphs and is well-known to be NP-hard. We use a classical polytime approximation to solve the problem within a factor of $2(1-1/|\tilde{\mathbf{S}}|)$, where $|\tilde{\mathbf{S}}|$ is the number of collapsed nodes resulting from the initial selection $\mathbf{S}$~\cite{KouSteinerApproximation}. After adding the necessary nodes to create a tree in the collapsed graph to the initial set of nodes $\mathbf{S}$, the connectivity subgraph $G_s$ is connected. 



% \parab{Modelling Sensor Heterogeneity.}
% With all the grid-based approximations, modeling heterogeneity becomes very straightforward and modular as follows. 

% \parae{ Heterogeneity in Sensor Types.} If the synthesis requires coverage by multiple types of sensors such as cameras and microphone, we can treat each sensor placement problem as a separate coverage problem. We can generate a separate visibility graph for each type ($t$) of the sensor, $G^t_v = (V, E^t_v)$ and solve the respecting k-vertex cover problem, followed by the connectivity repair method on the combined solution.

% \parae{ Heterogeneity in Sensor Capabilities.} 
% If the synthesis requires the placement of multiple sensors of the same type (e.g., camera) but with different specifications, we generate a separate visibility graph for each sensor specification ($t \in \{1, \cdots T\}$) as $G^t_v = (V, E^t_v)$. Then we can introduce a new Boolean $b_{t, j,z}$ to represent the placement of z-th type-t sensor in grid $j \in V$.
% \begin{equation}
% \label{hetero-sat}
% \begin{split}
%     &\bigwedge_{i\in V}\quad\left( \ \sum_{t = 1}^{T} \sum_{j \in \mathcal{N}_i(G^t_v)}   \ \  \sum_{z = 1}^{Z^t} b_{t, j,z} \geq k \right)\\
%     &\sum_{j = 1}^{|V|} \sum_{z = 1}^{Z^t} b_{t,j,z} = N^t  \ \ \ \forall t \in \{1, \cdots, T\}
% \end{split}
% \end{equation}
% where $N^t$ represents maximum number of sensor of type t, and $Z^t$ represent maximum number of type-t sensors allowed in same grid.  
% For connectivity, again, we can combine the solution and use the connectivity repair method.



\parab{The overall formulation.}
Summarizing our discussion so far, we can encode a MILP formulation of the k-coverage network synthesis goal with the following mapping of our four main constraints presented in \tabref{tab:prob_overall_sat}.



\begin{table}[!ht]
    \centering
    \caption{Summary of MILP Encoding of k-Coverage}
    % \resizebox{}{!}{
    {\begin{tabular}{ccc}
            \hline
        Coverage  & (C1)  &  k-Vertex Cover in Visibility Graph \\     
        Visibility & (C2)  &  Visibility Graph \\
        Connectivity & (C3)  &  Steiner Tree in Connectivity Graph\\ 
        Placement & (C4)  & Not Required\\ \hline
    \end{tabular}}
    % 
    \label{tab:prob_overall_sat}
\end{table}


% \begin{algorithm}[h!]
% \SetAlgoLined
% \KwResult{A set of locations $S*\subseteq\mathbf{U}$ describing a connected network with $S\subset S^*$.}
% \textbf{Input:} A subset of locations $S\subseteq\mathbf{U}$ and a connectivity graph $H$ as defined in Section \ref{conngraph}. \\
% Identify connected components in connectivity subgraph $H[S]$\\
% Map each component to a new ``collapsed" vertex \\
% Map edges of $H$ to their collapsed vertices \\
% Solve the Steiner tree problem on set of collapsed vertices corresponding to $S$ \\
% $S^* \leftarrow S\cup\{\text{vertices identified by Steiner tree result}\}$
% \caption{\label{connalg} Network connectivity enforcement}
% \end{algorithm}

%% \parab{Observations and Extensions.} To extend our SAT formulation to heterogeneous sensors with differing ranges, we can represent each vertex in the coverage graph via multiple Boolean variables, with each representing a different type of sensor. 

%% In addition to constraint flexibility and extensions to heterogeneous networks, the methodology allows for rapid re-planning.  Once the visibility and connectivity graphs corresponding to the discretized environment and sensor resources are formed, the construction of a SAT query is simple and lightweight, even for very large spaces.  This graph generation is also performed offline, meaning after once computation, any number of queries on the graph can be made with relative ease and speed, making reconfiguration and planning simple.

% The crux of this discretization lies on the generation of the bipartite graph, which requires $\frac{1}{2}|\mathbf{U}|^2$ number of computations for generating the graph. Since this is all done before invoking the SAT solver, we can take advantage of parallelization in modern computers for this. Additionally, this computation is required only once for an environment and sensor asset type (defined by its sensing radius), then any number of SAT queries can be made without recomputing the graph at each step.



==> reladed_work_J.tex <==
% Related work from Jonathan's digging

\section{Related Work (J)}

\begin{itemize}
	\item \cite{SATdisjointkcovers} : Solves the problem of dividing an existing deployment of sensors into the maximum number of disjoint k-covers.  Uses boolean SAT to solve a series of disjoint set cover subproblems and search for a maximum number of them.  I liked this paper because it uses similar terminology as far as coverage functions between sensors and regions, and discusses marriage of these concepts with SAT.  Paper is similar in this aspect, and because one of the subproblems they solve is the disjoint set cover problem  in SAT and we also solve this set cover problem using SAT in our formulation.
	
	\item \cite{MCLCT}: Solves the problem of finding maximum connected cover problem, deploying sensors to cover a set of DPOIs, where connectivity is only considered with respect to a central server.  Expresses several modifications/constraints and heuristics which can be handled to address various concerns with solutions to this problem such as loss of coverage, minimal sizes, and avoiding nodes playing both relay and sensing roles.  Optimizes sensor coverage subject to these constraints using a proposed algorithm/heuristic.  It also presents a probabilistic load balancing strategy which tries to evenly distribute transmission energy load among the various coverage trees.
	
	\item \cite{TrafficSchedPlace} : Solves simultaneous sensor placement and scheduling.  Exploits the submodularity of sensor placement's effect on coverage and increase in sensing quality (i.e. added sensors produce diminishing returns on quality of sensing and covered area) to allow for the use of greedy algorithms in submodular optimization. (I've actually implemented some of this in our problem if you guys are curious, they're very elegant and ridiculously fast)  Considers scheduling as a series of solutions to these problems, and solves simultaneous placement and scheduling as an alternating search in placement vs optimization on scheduling. Algorithm scales incredibly well, but oes not consider or worry about connectivity constraints and is generally fairly inflexible to constraints. (as a result of using a greedy algorithm.)
	
	\item \cite{WaterSensors} : Solves several example problems of selecting optimal placement of sensors in a water network with submodular objectives.  Considers a general penalty reduction scheme where the placement problem is cast as minimizing the expected reduction in penalty, where "penalty" is left generic so as to treat a variety of possible objectives.  Exploits the submodular optimization greedy algorithm which provides nice offline bounds and even tighter online bounds.  Does not consider many constraints aside from cardinality (number of sensors placed) but scales beautifully with runtime and optimality guarantees.
	
	\item \cite{DisjointKCover} : Also solves the disjoint set k-cover problem, where a set of sensors is already deployed and the goal is to identify disjoint sets to periodically activate.  They present some special variants of this problem where an entire set cover may not be desired and propose a greedy, randomized, and distributed algorithm to solve the problem with optimality guarantees. (with optimality being in the distance from the maximum number of set covers)  No flexibility to constraints or connectivity considered.
	
	\item \cite{LifetimePlacement} : Considers problem of minimizing the number of sensors required to cover a given set of target locations while maintaining a network lifetime of a certain guarantee.  Only considers connectivity to a base station and uses computational geometry tools for optimal placement in an obstacle-free environment.
	
	\item \cite{configurations} : Analyzes configurations and optimal lattice structures in free space to achieve coverage and connectivity for sensors.  Compares some normal deployment plans done in practice against the proposed optimal lattice structure.  Does not consider obstacles, but does consider connectivity and coverage and optimality in terms of number of sensors.
	
	\item \cite{FaultTolerant} : Addresses the problem of placing relay nodes to create k = 1, 2, and higher connectivity in both one and two way communication scenarios.  Only considers deploying relay nodes on top of a currently existing network.  Problem is proven to be NP-hard, and a series of polynomial approximation algorithms are presented to solve the problem for k = 1, 2 and a generalization is given for k > 2.
	
	\item \cite{RelayNodes} : Studies the two-tiered node placement for first coverage and then connectivity.  The idea for the two-tiered approach is for each sensor to be covered by relay nodes in order to communicate data.  These are the only constraints considered, addressing when sensing nodes need to be covered by both one and two relay nodes.  Connectivity with k = 1 and k = 2 is considered, but only with respect to base stations.
	
	\item \cite{DiscreteDiskCover} : Solves the discrete unit disk cover problem, or a ``sphere packing" problem.  Only tangentially related to our work, but provides some interesting context in WSN design.
	
	\item \cite{CentralizedandClustered} : Solves discrete set cover problem in an already-deployed network subject to connectivity constraints.  Each discrete set cover must be a connected network.  Is a protocol without using a general framework, so does not consider any other constraints.  Does not consider obstacles in the environment, uses a geometric approach to fill free space.
	
	\item \cite{UnifiedApproach} : A survey and attempt at combining various approaches towards solving sensor placement problem.  Considers a MILP/ILP formulation for various objectives such minimum number of placed sensors, and weighted coverage of a region.  Rather than a coverage/visibility graph, considers a coverage/visibility matrix which serves effectively the same purpose.  ILP methods allow for angle selection in placement, but examples with decent scalability only place < 10 sensors.
\end{itemize}

==> related_work_D.tex <==
% topics to cover here:
%density control
%cortez bullo (CB) alg
%extensions to CB for case with obstacles

\section{Related work (D)}

1) surveys : \cite{wang2011coverage},\cite{zhu2012survey}, \cite{al2017optimal}

2) optimal unconstrained deployment, highly cited, no sleep: \cite{bai2006deploying}

2) density control / sleep / activation / etc : \cite{xing2005integrated} \cite{zhang2005maintaining}

3) prior work in INFOCOM, other application-oriented papers: \cite{huang2014connected}



==> smt_backup.tex <==
\section{SMC Formulation of Network Synthesis}
\label{s:smc-form-netw}

%% In \secref{sec:proposed-sat}, we use a highly restricted discrete approximation of the  network synthesis problem to encode into a SAT problem. In this section, we present our second scalable approach for network synthesis where the amount of approximation is much less than the discrete SAT approach.

In this section, we leverage the recently-developed Satisfiability Modulo Convex (SMC) framework~\cite{shoukry2018smc} to formulate our network synthesis problem.

%% The contemporary paradigm of Satisfiability Modulo Convex (SMC) programming \cite{shoukry2018smc} provides an alternative approach for addressing the feasibility aspect of Mixed-Integer Convex problems with potentially improved efficiency and scalability. Instead of relying on relaxations of integer variables and branching, which is the starting point for many mixed integer algorithms, the SMC paradigm is based on a satisfiability approach.

%% \parab{Overview of SMC.}
%% SMC programming, designed to address the feasibility of mixed-integer convex problems, uses a SAT solver to suggest admissible assignments for a problem's Boolean variables\footnote{Note that one can almost trivially encompass integer variables via a larger number of Boolean variables, following the appropriate transformations.} and a convex solver to admissible values of the problem’s real variables. 
%% % Let us take the following example
%% % \begin{equation}
%% % \begin{split}
%% % \end{split}
%% %     a_1 \wedge (a_2 \vee a_3) \wedge (a_1 \rightarrow x_1 + x_2 = 4)
%% %     \label{eqn:satexample}
%% % \end{equation}
%% % Here, $a_1, a_2, a_3$ are Boolean variables and $x_1$,  $x_2$ are real variable. 
%% % The third clause implies that if $a_1$ is \textsc{True}, we should be able to find a valid value of $x_1$ and  $x_2$ such that $x_1 + x_2 = 4$ (convex constraint).
%% Potential infeasibilities in the convex constraints produce information (\textit{counter-examples}) that leads to a more efficient search over a more constrained solution space that excludes conflicting combinations of active constraints. The process is repeated until the suggested combination of convex constraints is satisfiable. 

%% Even if the theoretical worst-case complexity can be still approximately comparable to a complete enumeration, SMC-based solutions have been shown to perform better than earlier solution approaches to Mixed-Integer and other similar problems, especially for cases where the integer or Boolean variables and the respective constraints significantly outnumber the purely continuous part of the problem. Additionally, it is worth noting that the Boolean satisfiability formulas which one can use in the description of SMC problems can be more expressive than the typical syntax of Mixed-Integer convex problems, especially when it comes to complicated disjunctive formulas, without necessitating the use of relaxations (such as the ones reviewed in \cite{SIAM_MILP} for the Mixed-Integer Linear Programming case).

%% \begin{figure}[!ht]
%%     \centering
%%     \includegraphics[width=0.5\linewidth]{images/smc.png}
%%     \caption{Illustration of the SMC Process}
%%     \label{fig:smc}
%% \end{figure}

% The crux of SMC theory lies in the representation of a complex problem in terms of pseudo boolean constraints. 
% The constraints are presented in terms of Boolean or pseudo Boolean constrains. We incorporate the convex constraints and any complex constraints via the pseudo Boolean constraints. 
% -- add more info

\parab{Determining Coverage.} 
In our discretized space, we can approximate the problem of covering the entire area $\mathbf{L}$ by the problem of covering the corners of unoccupied grids.
Formally, let $\mathbf{L} = \bigcup_{u_i \in \mathbf{U}} \mathbf{L}^u_i$  where $\mathbf{L}^u_i$ denotes the four corners of the grid $u_i$.
Then, our formulation uses the following pseudo-Boolean variables to represent convex constraints:


\begin{table}[h]
    \centering
    \begin{tabular}{cccc}\hline
    		 & Pseudo   & & Respective   \\
		Description &Boolean & &  Predicate or \\
    					& Variable & & Constraints \\
            \hline
        Location Coverage  & $b^s_{ij}$  & $\rightarrow  $ &  $\mathcal{C}(s_i, l_j) $ \\     
        Grid Coverage  & $b^u_{ig}$  & $\rightarrow  $&  $\bigwedge_{l_j \in \mathbf{L}^u_g} \mathcal{C}(s_i, l_j)$ \\
        Visibility 	&  $b^o_{ijg}$   & $\rightarrow  $ &  $\mathcal{B}^o(s_i, l_j, o_g)$ \\
        Link Connectivity & $b^c_{ij}$   & $\rightarrow  $ &  $ \mathcal{P}(s_i, s_j) $\\ 
        Placement & $b^v_{ig}$   & $\rightarrow   $ & $\mathcal{V}^o\big(s_i,  o_g\big) $ \\ 
         \hline
    \end{tabular}
    % \caption{Caption}
    \label{tab:pseudo_bools}
\end{table}



%\begin{itemize}
%    \item $b^s_{ij}$ : if sensor $s_i$ can sense location $l_j \in \mathbf{L}$
%    \item $b^u_{ig}$ : if sensor $s_i$ can sense the entire grid area $u_g$
%    \item $b^c_{ij}$ : if sensor $s_i$ is connected to sensor $s_j$. $b^c_{ij} = b^c_{ji}$
%    \item $b^v_{ig}$ : if sensor $s_i$ is located outside of obstacles $o_g$
%    \item $b^o_{ijg}$ : if obstacle $o_g$ does not block the LOS between $s_i$ and location $l_j$ 
%    \end{itemize}

Using these, we can encode the problem into the SMC formulation as follows.


\parae{Visibility Constraints (C2).}
To express line-of-sight visibility, we use convex constraints described in \secref{sec:problem}: $\mathcal{B}(s_i, l_j) = \bigwedge_{o_g \in \mathbf{O}} \mathcal{B}^o(s_i, l_j, o_g)$  represents the condition that none of the obstacle $o_g \in \mathbf{O}$ obstruct the visibility between $s_i$ and $l_j$, resulting in:
\begin{equation}
    \psi_1 = \bigwedge_{i=1}^{N} \bigwedge_{l_j \in \mathbf{L}} \bigwedge_{o_g \in \mathbf{O}} \bigg(  b^o_{ijg}\rightarrow \mathcal{B}^o
    (s_i, l_j, o_g) \bigg)
\end{equation}



\parae{Coverage Constraints (C1).}
Our goal is to ensure that each grid region $u_g$ is covered by at least $k$ sensors:
\begin{equation}
    \psi_2 = \bigwedge_{u_g\in \mathbf{U}} \left( \sum_{i=1}^{N} b^u_{ig} \geq k \right) 
\end{equation}

However, covering a grid implies that the same sensor should cover all four corners of the grid, encoded as:
\begin{equation}
    \psi_3 = \bigwedge_{u_g\in \mathbf{U}} \left( b^u_{ig} \rightarrow   \bigwedge_{l_j\in \mathbf{L}^u_g} b^s_{ij} \right)
\end{equation}
which expresses the constraint that if sensor $s_i$ covers a grid $u_g$ ($b^u_{ig} = \textsc{True}$), then it covers all four corners of the grid $l_j\in \mathbf{L}^u_g$.

Now, to complete the representation, we need to represent the coverage of a location $l_j$ by a sensor $s_i$ (\eqnref{e:coverage}):
\begin{equation}
    \psi_4 = \bigwedge_{i=1}^{N} \bigwedge_{l_j \in \mathbf{L}}  \left( b^s_{ij} \rightarrow \bigg( \mathrm{dist}(s_i,l_j) \leq r^s_i \bigg) \bigwedge  \bigg( \bigwedge_{o_g \in \mathbf{O}} b^o_{ijg} \bigg) \right)
\end{equation}
%	This expresses the constraint that, for a sensor $s_i$ to cover a location $l_j$, the distance between them should be less than the coverage radius of the sensor $r_s$ and no obstacle should block the line of sight (LOS).


\parab{Connectivity Constraints (C3).}
Unlike the SAT formulation, we can easily encode network connectivity in the SMC formulation. In a connected network, there should exists a communication path (single hop or multihop) between every pair of nodes. Following the discussion in \secref{sec:problem}, a pair of nodes $s_i$ and $s_j$ is connected if they are within the communication radius:
\begin{equation}
    \psi_5 = \bigwedge_{i=1}^{N} \bigwedge_{j=1, j \neq i}^{N} \bigg( b^c_{ij} \rightarrow  \left(dist(s_i,s_j) \leq r^c_{i,j} \right) \bigg)
\end{equation}
Similarly, if $\hat{A}_h$ represents the $h$-hop adjacency matrix (whose $i,j$-th entry is the number of $h$-hop paths between $s_i$ and $s_j$), then we can write (\secref{sec:problem}):
\begin{equation}
     \psi_6 = \bigwedge_{j=2}^{N} \left( (\hat{\mathbf{A}}_N)_{1j} > 0 \right)
\end{equation}
In this formulation we have simplified the connectivity formulation:
we only check connectivity between node 1 and every other node because if there exists a path from node 1 to every other node, they can always connect via node 1.

\parab{Obstacles and sensor placement (C4).}
Finally, to make sure that the SMC solver does not put the sensor inside the obstacles, we add the following sets of clauses:
\begin{align}
    \psi_7 &= \bigwedge_{i=1}^{N}  \bigwedge_{o_g \in \mathbf{O}}  b^v_{ig} \\
 \psi_8 &= \bigwedge_{i=1}^{N}  \bigwedge_{o_g \in \mathbf{O}} \bigg(  b^v_{ig}\rightarrow \mathcal{V}^o(s_i, o_g) \bigg)
\end{align}
Here $\mathcal{V}^o(s_i, o_g) $ concisely represents the four convex constraints to represent the  placement outside of an obstacle $o_g$.

\parab{The overall formulation.}
Putting all these together, we arrive at the overall SMC formulation:  $\psi = \bigwedge_{i=1}^{8} \psi_i$.
With this formulation, we binary search of $N$ to find the solution with the fewest number of sensors.
Again, the four key constraints can be summarized as follows.
\begin{table}[h]
    \centering
    \begin{tabular}{ccc}
            \hline
        Coverage  & (C1)  &  $\psi_2$\\     
        Visibility & (C2)  &  $\psi_1 $ \\
        Connectivity & (C3)  & $\psi_6$\\ 
        Placement & (C4)  &  $\psi_7$\\ \hline
    \end{tabular}
    % \caption{Caption}
    \label{tab:prob_overall_smc}
\end{table}


%% we can vary the number of sensors $N$ from $k$ to maximum number of sensors available and stop when a feasible solution exists. The smallest value of $N$ with the feasible solution is our output. Secondly, we can do a binary search similar to the SAT based method to find the smallest feasible solution. 

%% Additional goal is to minimize the communication costs of the network. 


% \parab{Complete SMC Formulation.}
% The entire set of coverage constraints are as follows:
% \begin{equation}
% \begin{split}
%     \psi_1 &= \bigwedge_{u_g\in \mathbf{U}} \left( \sum_{i=1}^{N} b^u_{ig} \geq k \right) \ , \ \
%     \psi_2 = \bigwedge_{u_g\in \mathbf{U}} \left( b^u_{ig} \rightarrow   \bigwedge_{l_j\in \mathbf{L}^u_g} b^s_{ij} \right)\\
%     \psi_3 &= \bigwedge_{i=1}^{N} \bigwedge_{l_j \in \mathbf{L}} \left( b^s_{ij}\rightarrow \left(dist(s_i,l_j) \leq r^s_i \right) \wedge \left( \bigwedge_{o_g \in \mathbf{O}} b^v_{ijg}  \right) \right)
% \end{split}
% \end{equation}


% Now, the connectivity constraints can be represented as follows.
% \begin{equation}
% \begin{split}
%      \psi_4 &= \bigwedge_{i=1}^{N} \bigwedge_{j=1, j \neq i}^{N} \left( b^c_{ij} \rightarrow  \left(dist(s_i,s_j) \leq r^c_{i,j} \right) \right) \\
%      \psi_5 &= \bigwedge_{j=2}^{N} \left( \hat{A}_N)_{1j} > 0 \right)
% \end{split}
% \end{equation}

% Lastly, all the obstacle related constraints are as follows.

% \begin{equation}
% \begin{split}
%     \psi_6 &= \bigwedge_{i=1}^{N} \bigwedge_{j=1}^{M} \bigwedge_{o_g \in \mathbf{O}}  b^v_{ijg}\rightarrow \mathcal{B}(s_i, l_j, o_g) \\
%     \psi_7 &= \bigwedge_{i=1}^{N}  \bigwedge_{o_g \in \mathbf{O}}  b^o_{ig}\rightarrow \mathcal{V}(s_i, o_g) \\
%     \psi_8 &= \bigwedge_{i=1}^{N}  \bigwedge_{o_g \in \mathbf{O}}  b^o_{ig}
% \end{split}
% \end{equation}




\parab{Scaling Methods.} As discussed in \secref{s:netw-synth-appr}, SMC scales less well than SAT. We use three approaches to improve its scalability:  constraint pre-computation, hierarchical synthesis, and incremental coverage repair.

%% With the above formulation, it turns out that SMC scales up to a very small region of interest with very few ($5-8$) obstacles. 
%% However, for the range of problem it is scalable, the smallest feasible solution is around 2 times smaller than the SAT based encoding. To support scalability for much larger and complex problems, we first identify the reasons behind non-scalability: \emph{insufficient encoding of physical distance and large problem space. }

\parae{Constraint Pre-computation.} Recall that our SMC encoding discretizes the set of locations to be covered. If two such locations $l_i$ and $l_j$ are more than $2\cdot r^s$ distance apart (assuming sensor homogeneity with coverage radius of $r^s$ ), then no single sensor can cover them. While SMC can eventually determine this through counter-examples with our encoding, we have found that it significantly improves speed of synthesis to provide these as pre-computed constraints. We do this by (a) finding all pairs $l_i$ and $l_j$ that are greater than $2\cdot r^s$ distance apart and (b) adding a constraint that prevents a single sensor from covering them. (We add similar constraints for connectivity as well). 

%% One major issue with the above method is lack of proper encoding of physical distances between sensors. For example, in a symmetric network with sensing radius of $r_s$, if two sensed location is more than $2\cdot r_s$ distance apart, no sensor can sense both simultaneously. While the SMC method can figure these out via counter example generation, it takes much longer to identify all possible combinations. To circumvent, we precompute the pairwise distances between locations, identify the pairs with more than $2\cdot r_s$ distance, and add the necessary constraints. Similarly, in a symmetric network with communication radius of $r_c$, if two sensed location is more than $2\cdot r_s + r_c$ distance apart, two sensors that cover each of the location, can not communicate directly. Thus, there will not be any communication link between them. By adding such constraints, we are able to reduce the runtime and improve scalability. 

\parae{Hierarchical Synthesis.} To scale better, we subdivide the deployment area $\mathbf{L}$ into smaller sub-areas (\figref{fig:hiera_ilustration}) and solve for coverage (and not for connectivity) in each of the sub-areas separately. Then, once we have individual solutions, we need to connect them with each other so that we have a connected network.  
We could solve for both coverage and connectivity in each of the sub-areas. In complex deployment region, solving for both connectivity and coverage in each sub problem often over-provision the network. Also, the coverage solution itself mostly results in connected large sub-networks (\secref{sec:experiment}).

To connect the individual sub-problems, we can collapse each sub-area into a single node (Illustrated in \figref{fig:conn_reest}).  Then we can use constraints $\psi_4$ and $\psi_5$ in the SMC formulation to ensure connectivity between the sub-areas. In our evaluations (\secref{sec:experiment}), we label this approach \textit{SMC}.

%% However, for a larger number of nodes, the connectivity problem itself becomes intractable. In addition, we observe that the overall network is often already connected into smaller sub-networks, illustrated in \figref{fig:conn_reest:1}. 
%% With this we can collapse connectivity problem graph $G (V, E)$ into a smaller graph with its connected component $G' (V', E')$. Each node in $G'$ represents each connected component in G, illustrated in \figref{fig:conn_reest:2}.  This method is similar in a way to the SAT connectivity setup approach. 
%% We can now use this graph as a starting point for the connectivity problem.
\begin{figure}[!ht]
    \centering
    \includegraphics[width = \linewidth]{images/hierarchy.png}
    \caption{Illustration of Hierarchical Synthesis}
    \label{fig:hiera_ilustration}
\end{figure}

%In some cases, an alternative approach, labeled \textit{SMC-NoConn} scales better. In this approach, we solve only for coverage (and not for connectivity) in each sub-area.

%% Note that, for each subproblem, we can solve for a connected K-coverage or just K-coverage problem. While the first guarantees connectivity in each sub-problem, it might slightly overprovision in terms of overall solution. On the other hand, the second approach will likely to have less overprovisioning but might take more effort in the connectivity setup phase. In this paper, we compare both approach. For illustration, we will refer to the former as `SMC-Conn' and the later as `SMC-NoConn' approach. 

\parae{Incremental Coverage Repair.}
Hierarchical synthesis can help scaling but may result in redundant coverage, because each sub-area is solved independently, so parts of the area near the boundaries may be covered by more than $k$ sensors. To circumvent this, we first solve each sub-area for $k=1$ coverage. Then, for each grid element $d$, we measure the obtained coverage $k_d$ from this solution; grids near the boundary of each sub-area are likely to be covered by multiple sensors including those from neighboring sub-areas. The residual coverage requirement for $d$, then, is $k-k_d$; we now run the coverage problem again for each sub-area with these residual coverage requirements as constraints, which effectively ``fills'' up the coverage on grid points interior to the sub-area. After this, we apply the hierarchical connectivity determination described above.

%% propose another type of hierarchy: \emph{Coverage Hierarchy}. In this hierarchy, each subproblem is solve for $k$ coverage in two steps. First, we solve for a 1-coverage problem in each subproblem and combine the solution (without the connectivity step). Second, we evaluate the coverage level ($k_g$) of each grid $u_g \in \mathbf{U}$ with the combined solution. The required coverage level at $u_g$ is now $k-k_g$. Then, we run the hierarchical solver again but with the modified coverage requirements for each grid area ($k-k_g$). 
%% The solutions are combined and the connectivity step of Area Hierarchy is invoked to get the final solution.

\begin{figure}
    \centering
    % \subfloat[]{\label{fig:conn_reest:1}\includegraphics[width = 0.5\linewidth]{images/subnetwork.png}}
    \includegraphics[width = \linewidth]{images/collapsing.png}
    \caption{Illustration of Connectivity Restoring Method}
    \label{fig:conn_reest}
\end{figure}


%% \parab{Observations and Extensions.}
%% SMC approach can model complex problem with much simplicity compared to the SAT approach as well as other constrained optimization approaches. Moreover, it can be seen from the formulation that SMC can easily model heterogeneity of sensor into the formulation.
%% One can easily extend the encoding to include more complex sensing constraints such as: \emph{``each location should be covered by at least  2 cameras and 1 RF sensor.''}


==> story.tex <==

\section{Potential Infocom Story}
Three angles/steps of the story
\begin{enumerate}
    \item Given a set of requirements and a set of nodes, is it feasible to formulate a network?
    \item Given that the network is feasible, what is the optimal placement that contains the smallest number of devices? 
    Potential algorithms:
    \begin{enumerate}
        % \item Grid based Coverage and Spanning Tree Based Connectivity
        \item Grid based Coverage and SMC Based Connectivity
        \item Grid based Coverage and Connectivity
        \item SMC based Coverage and Connectivity in Grid Space
        \item SMC based Coverage and Connectivity in Continuous Space
        \item Hierarchical Approach for all of the above
    \end{enumerate} 
    \item For different ratios of sensing radius of $d_c$ and communication radius of $d_p$, how does the scalability of the proposed methods vary? Is there a way to identify the range of ratios for which each of the proposed methods are scalable?
    \item For different ratios of sensing radius of $d_c$ and deployment region dimensions, how does the scalability of the proposed methods vary? Is there a way to identify the range of ratios for which each of the proposed methods are scalable?
    \item What are the realistic values for sensing radius to communication radius ratios? What are the realistic values for sensing radius to deployment region dimension ratios?
\end{enumerate}


To get an idea of the practical values of these ratios: we need to estimate the real communication and sensing coverage range.
To get the coverage range for cameras: (1) test how many pixel does it takes to detect a face/person accurately? (2) Using the Camera Parameters estimate at max what distance can we get that many pixels for a human body/face.
(3) To get connectivity radius, either use the specs or manually estimate connectivity.

